Momentum-inspired Low-Rank Coordinate Descent for Diagonally Constrained SDPs

We present a novel, practical, and provable approach for solving diagonally constrained semi-definite programming (SDP) problems at scale using accelerated non-convex programming. Our algorithm non-trivially combines acceleration motions from convex optimization with coordinate power iteration and matrix factorization techniques. The algorithm is extremely simple to implement, and adds only a single extra hyperparameter -- momentum. We prove that our method admits local linear convergence in the neighborhood of the optimum and always converges to a first-order critical point. Experimentally, we showcase the merits of our method on three major application domains: MaxCut, MaxSAT, and MIMO signal detection. In all cases, our methodology provides significant speedups over non-convex and convex SDP solvers -- 5X faster than state-of-the-art non-convex solvers, and 9 to 10^3 X faster than convex SDP solvers -- with comparable or improved solution quality.

==> ICML20-AAAI21/AAAI-reviews.tex <==
Questions
1. {Summary} Please summarize the main claims/contributions of the paper in your own words. (Do not provide any review in this box)
This paper presents an accelerated coordinate descent-type method for solving SDPs with diagonal constraints. It provides theoretical guarantee on its local convergence rate and presents numerical results to demonstrate the effectiveness of the method.
2. {Novelty} How novel is the paper?
Paper contributes some new ideas
3. {Soundness} Is the paper technically sound?
I have not checked all details, but the paper appears to be technically sound
4. {Impact} How important is the paper likely to be, considering both methodological contributions and impact on application areas?
The paper will impact a moderate number of researchers
5. {Clarity} Is the paper well-organized and clearly written?
Excellent: paper is well organized and clearly written
6. {Evaluation} Are claims well supported by experimental results?
Moderate: Experimental results are weak: important baselines are missing, or improvements are not significant
7. {Resources} How impactful will this work be via sharing datasets, code and/or other resources? (It may help to consult the paper’s reproducibility checklist.)
Fair: some may find shared resources useful in future work
8. (Reproducibility) Would the experiments in the paper be easy to reproduce? (It may help to consult the paper’s reproducibility checklist.)
Good: e.g., code/data available, but some details of experimental settings are missing/unclear
9. {Reasons to Accept} Please describe the paper’s key strengths.
The paper provides a way to incorporate acceleration in the original Mixing Method and demonstrates its speed-up via numerical experiments.
10. {Reasons to Reject} Please describe the paper’s key weaknesses.
The paper builds heavily upon the work by Wang, Chang, and Kolter [WCK17], though WCK17 seems to be unpublished and the novelty of this paper will not be a serious issue if the authors are the same as those of WCK17. More critically, the analysis relies on the rather unnatural Assumption 4.1, which is non-standard in the SDP literature and certainly requires careful justification. Moreover, it is not convincing to claim the numerical efficiency of the proposed method based on comparison with general-purpose SDP solvers such as SeDuMi, SDPNAL+, and MoSeK. More careful comparisons with other first-order methods for SDP on wider range of problems are needed.
11. {Detailed Comments} Please provide other detailed comments and constructive feedback.
Major:
1) Assumption 4.1 is non-standard and unnatural. It seems that the assumption is made purely for technical convenience. However, this makes it difficult to compare the results in this paper against those in the literature and significantly weakens the theoretical contribution.
2) It is not fair to compare the proposed method with general-purpose interior-point SDP solvers. There are several other first-order methods for solving SDPs, such as
[1] Wen, Goldfarb, Scheinberg: Block Coordinate Descent Methods for Semidefinite Programming.
[2] Dang, Lan, Wen: Linearly Convergent First-Order Algorithms for Semidefinite Programming.
In particular, the RBR method in [1] is rather similar in spirit to the Mixing Method. As such, the authors should carefully explain the differences between the two.
3) To demonstrate the numerical superiority of the proposed method, I suggest that the authors conduct numerical experiments on more types of problems. One example is the MIMO detection problem from signal processing:
[3] Liu, Yue, So, Ma: A Discrete First-Order Method for Large-Scale MIMO Detection with Provable Guarantees.
Minor:
1) Line 48: The phase synchronization formulation in Boumal 2016 and Zhong and Boumal 2018 corresponds to M \rightarrow \infty, not general M. The cited references did not consider the quantized version.
2) Lemma 2.1: Actually, this result can already be found in the following paper from 1982:
Shapiro: Rank-Reducibility of a Symmetric Matrix and Sampling Theory of Minimum Trace Factor Analysis.
3) Line 167: Boumal 2016 did not discuss this rank result. The authors probably meant to refer to
Boumal, Voroninski, Bandeira: The Non-Convex Burer-Monteiro Approach Works on Smooth Semidefinite Programs.
12. {QUESTIONS FOR THE AUTHORS} Please provide questions for authors to address during the author feedback period. (Please number them)
Please address the issues raised in the detailed comments above.
=================================================
After reading the rebuttal, I still have doubts on the merits of the paper. From a theoretical perspective, the convergence result requires Assumption 4.1, which, as remarked in my review, is non-standard. It is not enough to just say that the assumption is satisfied in the numerical experiments, as SDPs are well known to have all sorts of degeneracies. Thus, the authors have not really addressed the core issue here. From a computational perspective, I agree with the other reviewer that the lack of comparison with other first-order methods is highly disappointing. Therefore, I will leave my score unchanged.
13. {Ethical Considerations} Please highlight any ethical considerations that must be considered before a final decision (it may help to consult the paper’s ethics statement, if provided)
N/A
14. (OVERALL SCORE)
4 - Reject
19. I acknowledge that I have read the author's rebuttal and made whatever changes to my review where necessary.
Agreement accepted
Reviewer #2
Questions
1. {Summary} Please summarize the main claims/contributions of the paper in your own words. (Do not provide any review in this box)
The paper present a new algorithm for solving diagonally constrained semi-definite programs (SDPs). It is based on the power iteration technique combined with a momentum gradient descent. The paper provides a convergence guarantee and a number of experiments on SDPs that are relaxations of the MaxCut and MaxSAT problem.
2. {Novelty} How novel is the paper?
Main ideas of the paper are known or incremental advances over past work
3. {Soundness} Is the paper technically sound?
I have not checked all details, but the paper appears to be technically sound
4. {Impact} How important is the paper likely to be, considering both methodological contributions and impact on application areas?
The paper will have low overall impact
5. {Clarity} Is the paper well-organized and clearly written?
Excellent: paper is well organized and clearly written
6. {Evaluation} Are claims well supported by experimental results?
Moderate: Experimental results are weak: important baselines are missing, or improvements are not significant
7. {Resources} How impactful will this work be via sharing datasets, code and/or other resources? (It may help to consult the paper’s reproducibility checklist.)
Poor: shared resources are not likely to be useful in future work
8. (Reproducibility) Would the experiments in the paper be easy to reproduce? (It may help to consult the paper’s reproducibility checklist.)
Excellent: e.g., code/data available and paper comprehensively describes experimental settings
9. {Reasons to Accept} Please describe the paper’s key strengths.
The paper is well-written and the theory seems sound. It provides a number of experiments.
10. {Reasons to Reject} Please describe the paper’s key weaknesses.
The paper proposes a new method for solving SDPs that have a bound constraint on the diagonal of the matrix. However, it does not provide a proper comparison to a very simple baseline: SDPs can be solved using the Burer-Monteiro factorization technique. An equality constraint on the diagonal can be easily included into the linear objective function via multiplying it with two diagonal scaling matrices. The resulting objective function is then not linear anymore but one just optimizes then a function subject to only a PSD constraint. Then, one can just apply any gradient descent scheme, either with a momentum or without, or with second-order correction like quasi-Newton or conjugate gradient descent. No need for a new algorithm then. This approach is basically also covered in [1]. It is not clear, that the proposed algorithm is faster than this approach. In some more fundamental way, they share a number of similarities.
algorithm in more detail:
let X = V'V
in each iteration:
v = norm of each colum-vector of V
perform one gradient/CG/quasi-Newton step of minimizing f(V) = <C, (V*diag(1/v))'(V*diag(1/v))>
Ref.
[1] Boumal, Nicolas. "A Riemannian low-rank method for optimization over semidefinite matrices with block-diagonal constraints." arXiv preprint arXiv:1506.00575 (2015).
11. {Detailed Comments} Please provide other detailed comments and constructive feedback.
The lack of comparison (in theory as well as in practice) to the simple approach described above is a major concern.
12. {QUESTIONS FOR THE AUTHORS} Please provide questions for authors to address during the author feedback period. (Please number them)
1. Why not use the simple approach as described above?
###################### Update after rebuttal ##################
After reading the authors' response I stick to rejecting the paper. The authors could not answer the question why they did not compare their algorithm to other simple, first order methods that make use of a factorization scheme. I was running the few lines of code that I provided above (and using an LBFGS solver) on the MaxCut problem and it is at least as fast as their new algorithm. Momentum terms have been used for non-linear optimization before.
14. (OVERALL SCORE)
3 - Clear reject
19. I acknowledge that I have read the author's rebuttal and made whatever changes to my review where necessary.
Agreement accepted
Reviewer #3
Questions
1. {Summary} Please summarize the main claims/contributions of the paper in your own words. (Do not provide any review in this box)
This paper combines acceleration motions, coordinate power iteration and matrix factorization techniques to present a practical approach for solving diagonally constrained SDPs. This algorithm is an improved version of Mixing Method, which only needs one parameter (similar to momentum). The experimental results show that this method has good experimental results in dealing with MaxCut and MaxSAT problems. At the same time, this paper logically and clearly proves that the method is locally linear convergence near the optimal solution.
2. {Novelty} How novel is the paper?
Paper contributes some new ideas
3. {Soundness} Is the paper technically sound?
I have not checked all details, but the paper appears to be technically sound
4. {Impact} How important is the paper likely to be, considering both methodological contributions and impact on application areas?
The paper will have a broad and significant impact
5. {Clarity} Is the paper well-organized and clearly written?
Good: paper is well organized but language can be improved
6. {Evaluation} Are claims well supported by experimental results?
Good: Experimental results are sufficient, though more analysis would significantly add support to the claims
7. {Resources} How impactful will this work be via sharing datasets, code and/or other resources? (It may help to consult the paper’s reproducibility checklist.)
Fair: some may find shared resources useful in future work
8. (Reproducibility) Would the experiments in the paper be easy to reproduce? (It may help to consult the paper’s reproducibility checklist.)
Good: e.g., code/data available, but some details of experimental settings are missing/unclear
9. {Reasons to Accept} Please describe the paper’s key strengths.
This article is technically sound and well written. The experiments also seem convincing.
10. {Reasons to Reject} Please describe the paper’s key weaknesses.
However, there are still some improvements to be made in this paper. I hope the following comments can be helpful to improve the paper:
1. It is particularly pointed out that the parameter \beta is very important, but the relevant experiments on the selection of \beta are ignored. Can we give the experimental results of choosing \beta?
2. There is a small problem. That is, Figure 1 and Figure 2 in the article are not clear.
3. In the reference paper [R1], the authors also solved the word embedding problem. As an improved algorithm of [R1], the problem is not solved in this paper because the result is poor? What are the reasons for the poor? It is hoped that the author will make a supplement.
[R1]Wang, P.-W.; Chang, W.-C.; and Kolter, Z. 2017. The Mixing method: coordinate descent for low-rank semidefinite programming. arXiv preprint arXiv:1706.00476.
11. {Detailed Comments} Please provide other detailed comments and constructive feedback.
1. It is particularly pointed out that the parameter \beta is very important, but the relevant experiments on the selection of \beta are ignored. Can we give the experimental results of choosing \beta?
2. There is a small problem. That is, Figure 1 and Figure 2 in the article are not clear.
3. In the reference paper [R1], the authors also solved the word embedding problem. As an improved algorithm of [R1], the problem is not solved in this paper because the result is poor? What are the reasons for the poor? It is hoped that the author will make a supplement.
[R1]Wang, P.-W.; Chang, W.-C.; and Kolter, Z. 2017. The Mixing method: coordinate descent for low-rank semidefinite programming. arXiv preprint arXiv:1706.00476.
12. {QUESTIONS FOR THE AUTHORS} Please provide questions for authors to address during the author feedback period. (Please number them)
However, there are still some improvements to be made in this paper. I hope the following comments can be helpful to improve the paper:
1. It is particularly pointed out that the parameter \beta is very important, but the relevant experiments on the selection of \beta are ignored. Can we give the experimental results of choosing \beta?
2. There is a small problem. That is, Figure 1 and Figure 2 in the article are not clear.
3. In the reference paper [R1], the authors also solved the word embedding problem. As an improved algorithm of [R1], the problem is not solved in this paper because the result is poor? What are the reasons for the poor? It is hoped that the author will make a supplement.
[R1]Wang, P.-W.; Chang, W.-C.; and Kolter, Z. 2017. The Mixing method: coordinate descent for low-rank semidefinite programming. arXiv preprint arXiv:1706.00476.
14. (OVERALL SCORE)
7 - Accept
Reviewer #4
Questions
1. {Summary} Please summarize the main claims/contributions of the paper in your own words. (Do not provide any review in this box)
This paper studies fast algorithms for the semidefinite programming problem (SDP) where only the diagonal elements are constrained. These diagonal-constrained SDPs arise as a continuous relaxation of combinatorial optimization problems such as MAXCUT and MAXSAT. A simple algorithm is provided that performs faster than the state of the art for MAXCUT on multiple benchmarks.
2. {Novelty} How novel is the paper?
Paper contributes some new ideas
3. {Soundness} Is the paper technically sound?
I have not checked all details, but the paper appears to be technically sound
4. {Impact} How important is the paper likely to be, considering both methodological contributions and impact on application areas?
The paper will have low overall impact
5. {Clarity} Is the paper well-organized and clearly written?
Good: paper is well organized but language can be improved
6. {Evaluation} Are claims well supported by experimental results?
Good: Experimental results are sufficient, though more analysis would significantly add support to the claims
7. {Resources} How impactful will this work be via sharing datasets, code and/or other resources? (It may help to consult the paper’s reproducibility checklist.)
Not applicable: no shared resources
8. (Reproducibility) Would the experiments in the paper be easy to reproduce? (It may help to consult the paper’s reproducibility checklist.)
Meets Minimum Standard: e.g., code/data unavailable, but paper is clear enough that an expert could confidently reproduce
9. {Reasons to Accept} Please describe the paper’s key strengths.
A simple algorithm is provided that performs faster than the state of the art for MAXCUT on multiple benchmarks. Thorough experiments.
10. {Reasons to Reject} Please describe the paper’s key weaknesses.
The main application seems (MAXCUT) seems somewhat limited. (Results on the other application, MAXSAT lag behind other methods on some important benchmarks.
#######Post Rebuttal########
I find the concerns raised by the expert reviewers significant and am changing the score accordingly.
11. {Detailed Comments} Please provide other detailed comments and constructive feedback.
For diagonal-constrained SDPs, Wang et al., 2017 gave a coordinate descent algorithm Mixing Method, which they showed to have favorable performance in experiments in addition to analyzing it theoretically. The present paper seeks to speed up this algorithm via momentum methods. It's not immediately clear how to apply the standard Polyak momentum method here which is normally applied to gradient-based methods. The main idea of the present paper is to adapt the acceleration idea of De et al., 2018 which applies to power iteration for PCA, to the mixing method of Wang et al., 2017.
12. {QUESTIONS FOR THE AUTHORS} Please provide questions for authors to address during the author feedback period. (Please number them)
k is set to \sqrt{2n}. Doesn't this invalidate the analysis due to Goemans--Williamson for the approximation factor achieved by their SDP relaxation of MAXCUT. Goemans--Williamson do not have any rank assumptions as far as I know. Perhaps, for k restricted as here, one can show that for certain classes of graphs the analysis of Goemans--Williamson still applies?
14. (OVERALL SCORE)
4 - Reject
19. I acknowledge that I have read the author's rebuttal and made whatever changes to my review where necessary.
Agreement accepted
Reviewer #5
Questions
1. {Summary} Please summarize the main claims/contributions of the paper in your own words. (Do not provide any review in this box)
The algorithm Mixing Method ++ proposed in the paper is new. It can be viewed as an extension of the Mixed Method in which some sort of acceleration is added. Its analysis seems to be quite similar to the one for the Mixing Method though. The fact that its convergence is established only for the situation in which the initial point is close to the set of optimal solutions is a drawback in my opinion. I would like to see a result that shows that the generated sequence converges to some point satisfying first (and possibly second) order necessary conditions. There are many convergence results that have been obtained, under some probabilistic assumption on the data, for low-rank methods showing that they converge to the global solution regardless of the initial point choice (see for example Boumal et al, The nonconvex Burer-Monteiro approach works on smooth semidefinite programs, Advances in Neural Information Processing Systems, 2757-2765, 2016). Another drawback is that there is no discussion relating the method proposed in the paper with the types of results obtained in the aforementioned paper (and others of similar type). Another negative aspect of the Mixing M++ is that it is designed to solve only diagonally constrained SDPs rather than general ones. In summary, the algorithm is new but its applicability and the theoretical results derived for it are limited in scope.
The numerical performance of Mixing M. ++ seems to be excellent. However, the authors directly compare it to codes that do not take advantage of the simple form of max cut SDP feasible region. For example, SDPLR is designed for solving any SDP and uses an augmented Lagrangian approach to obtain a near feasible solution in the limit. However, using the ideas developed in Burer and Monteiro (OMS 15, pages 175-200, 2001), it is possible to easily implement a more specialized version of SDPLR which forces every iterate to be feasible and that should substantially improve its performance. (Currently, I am not sure whether SPPLR takes advantage of the simple structure of the max cut SDP problem. In summary, the numerical results of the paper would be more convincing if the authors could compare their method with more specialized methods that specifically take advantage of the simple form of the max cut SDP relaxation problem.
The paper is worth publication particularly in view of its numerical results but this reviewer does not believe it to be up to the standard of AAAI unless a great part of the above criticism is addressed.
2. {Novelty} How novel is the paper?
Paper contributes some new ideas
3. {Soundness} Is the paper technically sound?
I have not checked all details, but the paper appears to be technically sound
4. {Impact} How important is the paper likely to be, considering both methodological contributions and impact on application areas?
The paper will have low overall impact
5. {Clarity} Is the paper well-organized and clearly written?
Good: paper is well organized but language can be improved
6. {Evaluation} Are claims well supported by experimental results?
Good: Experimental results are sufficient, though more analysis would significantly add support to the claims
7. {Resources} How impactful will this work be via sharing datasets, code and/or other resources? (It may help to consult the paper’s reproducibility checklist.)
Not applicable: no shared resources
8. (Reproducibility) Would the experiments in the paper be easy to reproduce? (It may help to consult the paper’s reproducibility checklist.)
Good: e.g., code/data available, but some details of experimental settings are missing/unclear
9. {Reasons to Accept} Please describe the paper’s key strengths.
Numerical results seem to be quite solid but more convincing
10. {Reasons to Reject} Please describe the paper’s key weaknesses.
The paper is incomplete as it is (see my comment previous comments above).
11. {Detailed Comments} Please provide other detailed comments and constructive feedback.
The quality of the paper can certainly be improved if the authors could address the comments above.
12. {QUESTIONS FOR THE AUTHORS} Please provide questions for authors to address during the author feedback period. (Please number them)
I would like to see the negative comments about the theoretical results and the implementation results addressed.
14. (OVERALL SCORE)
3 - Clear reject
19. I acknowledge that I have read the author's rebuttal and made whatever changes to my review where necessary.
Agreement accepted
Meta Review:
3. Detailed Comments (Please also summarize discussion on this paper)
The reviewers of this paper were divided on the quality of this work. There is general agreement that the paper has some merits but also some notable shortcomings.
The primary concerns about the paper are,
- The required Assumption 4.1, which is non-standard and not required by other SDP methods.
- The experiments lack a direct comparison to other state-of-the-art first order methods.
Addressing these points would require major changes to the proposed work and hence it cannot be published in its current form.

==> ICML20-AAAI21/ICML_experiments.tex <==
\section{Experimental Results}
There are two well-known applications of our objective in \eqref{eq:continuous_form}: MaxCut and MaxSAT. 
We use the same formulation in \cite{wang2017mixing} to solve those two problems by continuous relaxation. 
We implement \texttt{Mixing Method++} in C with $\beta=0.8$ \footnote{We have performed empirical hyperparameter tuning to test our theoretical bound; after testing a group of values from the set $[0,1)$ with step size $0.01$, $\beta = 0.8$ yields the best performance (on average and) on above 90\% of instances.}  and compare it with a group of SDP solvers that can solve both MaxCut and MaxSAT formulations, as well as dedicated MaxSAT solvers. 
In addition to these applications, we provide experiments on the MIMO signal detection objective \cite{liu2017discrete}, further demonstrating the superiority of \texttt{Mixing Method++}.
Each experiment is run on a single core in a homogeneous Linux cluster. 
Each core is at 2.63 GHz with 16 GB of RAM.

\subsection{MaxCut}
\begin{table*}
\centering
\begin{small}
\begin{tabular}{ccccccc}
\toprule
Solver  & & \# Solved instances & &  median(log(objective residual)) & & Acceleration ($\times$) \\ 
\cmidrule(lr){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} 
Sedumi  & & 60  & & -4.30 & & 360.20 \\ 
MoSeK   & & 74  & & -3.24  & & 348.37  \\ 
SDPNAL+ & & 52  & & \textbf{-4.33} & & 1316.35 \\ 
CGAL &  & 92  &  & 0.93 & & 49.19 \\ 
SDPLR & & 95 &  & -2.89 &  & 9.14  \\ 
Mixing Method  & & 106 & & -2.80 & & 5.26 \\ 
\texttt{Mixing Method++} & & \textbf{111} & & -3.87 & & \textbf{1} \\ 
\bottomrule
\end{tabular}
\end{small}
\caption{\small \textbf{Results on 203 MaxCut instances.}  \texttt{Mixing Method++} solved most instances efficiently with decent precision. E.g., \texttt{Mixing Method++} is 5.26 and 360.20 times faster than Mixing Method and Sedumi, respectively. The median of log(objective residual) of \texttt{Mixing Method++} is -3.87, meaning that the median precision of \texttt{Mixing Method++} on all cases is $10^{-3.87}$.} \label{table:maxcut}
\end{table*}

The SDP relaxation of MaxCut problem is:
\begin{equation*}
     \underset{\|v_i\|=1,}{\mathrm{max}}\,\tfrac{1}{2}\sum_{ij}c_{ij}\left(\tfrac{1-v_i^\top v_j}{2}\right),
\end{equation*}
where $C$ is the adjacency matrix.
Thus we minimize the following objective function $f_{\text{MaxCut}}$:
$$
 f_{\text{MaxCut}} = \left\langle\tfrac{\mathds{1}_{n \times n}- V^\top V}{4} , C \right \rangle,
$$
where $\mathds{1}_{n \times n}$ is the $n\times n$ matrix with $1$ on every entry.
We consider the following two sets of benchmarks.
\vspace{-0.2cm}
\begin{itemize}[leftmargin=*]
    \item  Gset: 67 binary-valued matrices, generated by an autonomous random graph generator. The dimension $n$ varies from $800$ to $10^4$. \vspace{-0.2cm}
\item Dimacs10: This benchmark consists of 152 symmetric matrices (with $n$ varying from $39$ to $50,912,018$) chosen for the $10$th Dimacs Implementation Challenge.  We consider the 136 datasets with dimension $n \le 8\cdot 10^6$. \vspace{-0.2cm}
\end{itemize}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{ICML_exps/time-eps-converted-to.pdf} \vspace{-0.6cm}
\caption{\textbf{CPU time vs Size on MaxCut.} We run all SDP solvers with time limit 24h ($8.64\times 10^4$s). \texttt{Mixing Method++} solves most cases and is the fastest solver.}
\label{exp:maxcut_time}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=1\columnwidth]{ICML_exps/error-eps-converted-to.pdf} \vspace{-0.6cm}
\caption{\textbf{Objective residual vs size on MaxCut.} \texttt{Mixing Method++} shows at least competitive performance. As an approximate method, CGAL has large objective residual.}
\label{exp:maxcut_error}
\end{figure}


\begin{figure}[h!]
\centering
\includegraphics[width=1.1\columnwidth]{ICML_exps/ICML_maxcut_G40.pdf}  \vspace{-0.6cm}
\caption{\textbf{G40: $n=2000$, number of edges $ = 11766$.} \texttt{Mixing Method++} converges within $1$s while Mixing Method uses about $4$s. MoSeK and Sedumi need $10^2$ and $10^3$ seconds respectively to converge.} 
\label{exp:maxcut_G40}
\end{figure}

\vspace{-0.1cm}

\begin{figure}[h!]
\centering
\includegraphics[width=1.1\columnwidth]{ICML_exps/ICML_maxcut_uk.pdf}  \vspace{-0.6cm}
\caption{\textbf{uk: $n=4824$, number of edges$ = 6837$.} Consider the CPU time when each solver reaches objective residual $10^{-2}$. \texttt{Mixing Method++} uses only 20s while Mixing Method needs 200s. MoSeK and Sedumi consume more than $10^3$ and $10^4$ seconds respectively.}
\label{exp:maxcut_uk}
\end{figure}

 

We compare \texttt{Mixing Method++} with:
\begin{itemize}[leftmargin=*]
\item CGAL \cite{CGAL}, a provably correct algorithm for solving large SDP problems by matrix sketching. We set rank $R=\lceil\sqrt{2n}\rceil$.  \vspace{-0.1cm}
\item Sedumi \cite{sturm1999using}, a package for optimization problems with linear, quadratic and semidefinitness constraints by self-dual embedding technique.  \vspace{-0.1cm}
\item SDPNAL+ \cite{yang2015sdpnal}, a  Newton-CG augmented Lagrangian method for SDP. \vspace{-0.1cm}
\item SDPLR \cite{burer2003nonlinear}, a low-rank method using L-BFGS on the extended Lagrangian problem. \vspace{-0.1cm}
\item MoSeK \cite{aps2019mosek}, a software package to solve large scale sparse problems. \vspace{-0.1cm}
\item Mixing Method \cite{wang2017mixing} (Algorithm  \ref{algo:mixing}), state of the art solver for unit diagonal SDP. \vspace{-0.1cm}
\end{itemize}


We set the stopping criterion of \texttt{Mixing method++} and Mixing Method to $10^{-5}$, the rank $k$ to $\lceil\sqrt{2n}\rceil$, and use default setting for other methods. 

We plot CPU time in Figure \ref{exp:maxcut_time} and \textbf{objective residual} (the difference between objective value given by a solver and the lowest objective value from all solver's outputs.) 
Let $\texttt{Obj}_{ij}$ be the value of the objective function given by optimizer $i$ on instance $j$, the objective residual is defined by $|\texttt{Obj}_{ij}-\mathop{\min}\limits_{i'\in O}\texttt{Obj}_{i'j}|$ where $O$ is the set of all optimizers.

In Figure \ref{exp:maxcut_error}, \texttt{Mixing Method++} has the best performance in terms of CPU time and maintains high quality solution in the sense of it yields low objective residual.

More quantitatively, Table \ref{table:maxcut} lists the number of solved instances, median logarithm of objective residual, as well as the pairwise acceleration ratio.\footnote{When a instance is solved within time limit by \texttt{Mixing Method++} and solver $s$, the pairwise acceleration ratio is the ratio of CPU time of solver $s$ and that of \texttt{Mixing Method++}.}  For all 203 instances, within 24 hours, \texttt{Mixing Method++} solved most instances (111) among all solvers, \emph{and is $5\times$ to $1316\times$ faster than other solvers.} 
Moreover, the efficiency of \texttt{Mixing Method++} does not harm its precision. 
Our method achieves the median logarithm objective residual of $-3.87$, which is preceded only by Sedumi (-4.30) and SDPNAL+ (-4.33). However, both of those two solvers are more than $300\times$ slower than \texttt{Mixing Method++}.

We also study two specific cases of MaxCut, \texttt{G40} from Gset and \texttt{uk} from Dimacs10. In Figure \ref{exp:maxcut_G40} and \ref{exp:maxcut_uk}, we plot the objective residual of \texttt{Mixing Method++} and other SDP solvers to show the speed of convergence.\footnote{We do not include CGAL and SDPLR in the plots. The reason is the intermediate solution given by those methods is infeasible, turning intermediate objective values hard to interpret and quantify.} In both MaxCut instances, \texttt{Mixing Method++} converges significantly faster than MoSeK and Sedumi. When compared with Mixing Method, our method might converge slightly slower at an early stage but is able to catch up quickly.


\subsection{MaxSAT}

% \begin{table*}
% \centering
% \begin{small}
% %\resizebox{.5\textwidth}{!}{
% \begin{tabular}{ccccccccc}
% \toprule
% \multicolumn{1}{c}{Methods} & & \multicolumn{1}{c}{Crafted (331)} & & \multicolumn{1}{c}{Random (454)} & &  \multicolumn{1}{c}{Industrial (65)} & & \multicolumn{1}{c}{Total (850)} \\ 
% \cmidrule(lr){1-1} \cmidrule(lr){3-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7} \cmidrule(lr){9-9} 
% % \midrule
% \multicolumn{1}{c}{Loandra} & & \multicolumn{1}{c}{0.918} & & \multicolumn{1}{c}{0.957}  & & \multicolumn{1}{c}{\textbf{1}} & & \multicolumn{1}{c}{0.945} \\ 
% \multicolumn{1}{c}{Mixing Method} & &  \multicolumn{1}{c}{\textbf{0.999}} & & \multicolumn{1}{c}{\textbf{0.996}} & & \multicolumn{1}{c}{0.713} & & \multicolumn{1}{c}{0.975} \\ 
% \multicolumn{1}{c}{\texttt{Mixing Method++}} & & \multicolumn{1}{c}{\textbf{0.999}} & & \multicolumn{1}{c}{\textbf{0.996}} & & \multicolumn{1}{c}{0.731} & & \multicolumn{1}{c}{\textbf{0.977}}      \\ \bottomrule
% \end{tabular}
% %}
% \end{small}
% \caption{\textbf{Results on MaxSAT.} Overall, \texttt{Mixing Method++} achieves the best approximate ratio (0.977).  Time limit = 300s.}
% \label{table:maxsat}
% \end{table*}

\begin{table}
\centering
\begin{small}
%\resizebox{.5\textwidth}{!}{
\begin{tabular}{ccc}
\toprule
\multicolumn{1}{c}{Methods} & & \multicolumn{1}{c}{Avg. Approx. Ratio} \\ 
\cmidrule(lr){1-1} \cmidrule(lr){3-3}
% \midrule
\multicolumn{1}{c}{Loandra} & & \multicolumn{1}{c}{0.945} \\ 
\multicolumn{1}{c}{Mixing Method} & & \multicolumn{1}{c}{0.975} \\ 
\multicolumn{1}{c}{\texttt{Mixing Method++}} & & \multicolumn{1}{c}{\textbf{0.977}} \\ \bottomrule
\end{tabular}
%}
\end{small}
\caption{Results on MaxSAT. \texttt{Mixing Method++} achieves the best approximation ratio with a time limit of 300s. 850 problems are tested in total. Problems are derived from several domains, including crafted problems (331), random problems (454), and industrial problems (65).}
\label{table:maxsat}
\end{table}

Let $s_{ij}\in\{\pm 1,0\}$ be the sign of variable $i$ in clause $j$. The problem below provides an upper bound on the exact  MaxSAT solution: \vspace{-0.05cm}
$$
\underset{\|v_i\|=1,}{\mathrm{max}} \sum_{j=1}^m\left(1-\tfrac{\|Vs_j\|^2-(|s_j|-1)^2}{4|s_j|}\right), \vspace{-0.05cm}
$$
where $s_j=[s_{1j},...s_{nj}]^\top$.
Therefore, we minimize the following objective function for MaxSAT SDP relaxation:
$$
f_{\text{MaxSAT}} = \left\langle{V^\top V}, C \right \rangle, \quad \text{where $C=\sum_{j=1}^m\tfrac{s_js_j^\top}{4|s_j|}$.}
$$
We gather 850 instances from MaxSAT competition 2016-2019.
%\footnote{We excluded MaxSAT cases with hard clauses. The reason is, in those cases, a feasible assignment should firstly satisfy all the hard clauses, which is non-trivial for SDP-based methods.} 
The benchmarks are categorized into three tracks: \emph{random, crafted} and \emph{industrial}.
We used \texttt{Mixing Method++} as a partial MaxSAT solver. A partial solver only provides the assignment it finds with least number of violated clauses while a complete solver must give a proof of optimality.

We compare our method with the Loandra \cite{loandra}, the best partial solver in MaxSAT Competition 2019, and Mixing Method.
%\footnote{We do not include linear programming (LP) since \cite{wang2017mixing} shows LP relaxation for MaxSAT is outperformed by Mixing Method.}.
The average approximation ratio of each solver across all tested problem instances is shown in Table \ref{table:maxsat}.
% The results of approximation ratio of each solver is shown in Table \ref{table:maxsat}.
For cases where the optimal solution is not known, we use the best solution given by all solvers as ground truth.
\texttt{Mixing Method++} achieves the best average approximation ratio across problem instances.
% We achieved an average
% approximation ratio of 0.977. According to the experimental results of \cite{wang2017mixing}, Mixing Method performs well on random and crafted benchmarks but is unsatisfactory on industrial instances with large number of variables and clauses.  Compared with the Mixing Method, \texttt{Mixing Method++} improves the approximation ratio from 0.71 to 0.73  for these cases. Figure \ref{exp:maxsat_ind} shows the cost of solution of each solvers given time limit 300s.
In Figures \ref{exp:maxsat_s3v} and \ref{exp:maxsat_wb}, we plot the objective residual and cost (number of unsatisfied clauses) on two specific MaxSAT instances, \texttt{s3v90c800-6} from random track and \texttt{wb.4m8s4.dimacs.filtered} from  industrial track.
Our method outperforms Mixing Method in terms of convergence.
On the first instance, \texttt{Mixing Method++} returns the best solution of the three solvers.
On the industrial instance, Loandra provides the optimal solution quickly, but our method still produces a better solution than Mixing Method.

\begin{figure}[h!]
\centering
\includegraphics[width=1.1\columnwidth]{ICML_exps/ICML_maxsat_all.pdf} \vspace{-0.5cm}
\caption{\textbf{MaxSAT: cost of solution (time limit $ = 300$s).} Though Loandra, the champion of MAXSAT 2019 is the  best solver for large industrial instances, \texttt{Mixing Method++} improves the quality of solution compared to Mixing Method.}
\label{exp:maxsat_ind}
\end{figure}


\begin{figure}[h!]
\centering
\includegraphics[width=1\columnwidth]{ICML_exps/ICML_maxsat_s3v.pdf} \vspace{-0.5cm}
\caption{\textbf{s3v90c800-6.cnf ($n=90$, $m=800$).} \texttt{Mixing Method++} not only converges faster than Mixing Method, but provides better solution (30) compared to Mixing Method (31) and Loandra (33). The optimal solution has cost 26.}
\label{exp:maxsat_s3v}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=1\columnwidth]{ICML_exps/ICML_maxsat_web.pdf} \vspace{-0.5cm}
\caption{\textbf{wb\_4m8s4\_dimacs\_filtered.cnf ($n=463,080$, $m=1,759,150$).} Loandra reaches optimal (230) in 1 sec, while Mixing Method and \texttt{Mixing Method++} return a solution with cost $28,306$ and $25,210$ respectively in 1 hour.}
\label{exp:maxsat_wb}
\end{figure}

% \begin{table}[]
%     \centering
%     \begin{tabular}{cc}
%          Methods &  Total Approx. Ratio \\
%          \midrule
%          Loandra & 0.945 \\
%          Mixing Method & 0.975 \\
%          \texttt{Mixing Method++} & \textbf{0.977}\\
%     \end{tabular}
%     \caption{Rresults on MaxSAT. \texttt{Mixing Method++} achieves the best approximation ratio with a time limit of 300s. 850 problems are tested in total. Problems are derived from several domains, including crafted problems (331), random problems (454), and industrial problems (65).}
%     \label{exp:maxsat_wb}
% \end{table}

\subsection{MIMO}
We also consider the MIMO signal detection setting given by the following problem.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/mimo_mm.pdf}
    \caption{Performance comparison of Mixing Method (dashed lines) and Mixing Method++ (solid lines) on the MIMO signal detection problems. Subplot titles denote the size of the problem (i.e., the value of $m \times n$), while line colors denote different signal-to-noise ratios. The top row is plotted in terms of iterations, while the bottom row is plotted with respect to CPU time.}
    \label{fig:mimo_mm}
\end{figure}

\begin{equation}
        \argmin\limits_{x \in \mathcal{S}} \|y - Hx\|_2^2\\
        \label{mimo_obj}
\end{equation}

In \eqref{mimo_obj}, $y \in \mathbb{R}^m$ is the signal vector, $H \in \mathbb{R}^{m \times n}$ is the channel matrix, and $x \in \mathcal{S}$ is the transmitted signal.
It is assumed that $y = Hx + v$, where $v \sim \mathcal{N}(0, \sigma_v^2)$.
%\footnote{The signal-to-noise ratio (SNR) of the MIMO detection problem can be modified by changing the variance $\sigma_v^2$ with which the noise vector $v$ is generated.}
For our experiments, $\mathcal{S} = \{\pm1\}^n$ because we consider the constellation for our transmitted signal to be $\{\pm1\}$.
By considering our constellation as such, \eqref{mimo_obj} can be reformulated into the following non-convex SDP.

\begin{equation}
    \min\limits_{V \in \mathbb{R}^{k \times (n+1)}} \langle L, V^TV \rangle ~\text{  s.t. } \|V_{:, i}\|_2 = 1 ~~\forall i
    \label{sdp_mimo}
\end{equation}

where $L = \begin{bmatrix} H^TH & -H^Ty \\ -y^TH & y^Ty\end{bmatrix}$ is our symmetric cost matrix within the space $\mathbb{R}^{(n + 1) \times (n + 1)}$.
We compare Mixing Method++ to the Mixing Method on several simulated instances of the MIMO SDP objective.
In all cases, $H$ is sampled i.i.d. from a standard normal distribution and each coordinate of $x$ is sampled independently from the constellation $\{\pm1\}$.
Our noise vector $v$ is sampled from a centered normal distribution with variance $\sigma_v^2$.
Experiments are performed for numerous different settings of $\sigma_v^2$, determined by the signal-to-noise ratio (SNR) (i.e.,  $\sigma_v^2 = \frac{mn}{\text{SNR}}$).
More specifically, we perform tests for $\text{SNR} \in \{8, 16\}$ with problem sizes of $(m, n) \in \{(16, 16), (32, 32), (64, 32)\}$.
The performance of Mixing Method++ in comparison to the Mixing Method is displayed in Fig. \ref{fig:mimo_mm}.
As can be seen, the performance of Mixing Method++ matches or exceeds the performance of the Mixing Method with respect to both iterations and wall-clock CPU time in all experimental settings that were explored, where we set $\beta = 0.4$.


\subsection{Sparsity Effect}
We here seek to compare the acceleration of Mixing Method++ for different sparsity levels, i.e., the number of zero-valued elements over the total number of elements. We conjecture that the advantage of Mixing Method++ to Mixing Method is more significant for sparser matrices $C$. In Figure.~\ref{fig:sparsity}, we investigate the MaxCut problem for a graph with size $n=500$. We consider adjacency matrices with three sparsity levels $0.8,0.5,0.2$ and plot the objective residual of MM and MM++ with the default momentum value $\beta=0.8$ for each case. To have a fair comparison, we first consider a fully-connected weighted adjacency matrix and then remove edges to have the three desired matrices. As shown in Figure~\ref{fig:sparsity}, the acceleration of MM++ is more significant for sparser matrices $C$. Decreasing the momentum value $\beta$ for more dense matrices $C$ helps to boost the performance of MM++.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/sparsity.pdf}
    \caption{Convergence comparison of Mixing Method++ (blue line) with $\beta=0.8$ and Mixing Method (orange line) on MaxCut problem for a set of $n=500$ nodes with three different adjacency matrices $C$. The sparsity values are respectively $0.8, 0.5, 0.2$ from left to right.}
    \label{fig:sparsity}
\end{figure}

\subsection{Adaptive Momentum Schedule}
Complied to the proposed experiments, MM++ is shown to converge faster than MM given even with the suggested momentum value $\beta=0.8$ (default). However, MM decreases the objective cost faster in the beginning, according to the observations. Furthermore, several recent works~\cite{o2015adaptive,chen2019demon,wang2020scheduled} have shown the advantages of an adaptive momentum compared to a fixed parameter. Inspired by this behavior, we suggest the use of a scheduled increasing momentum instead of a constant value; this way, we take advantage of a hybrid performance with a faster convergence. We indeed proposed to increase the momentum parameter $\beta$ from $0$ to some value $\beta_0$ where in our default case $\beta_0=0.8$. An exponential momentum schedule such as \mbox{$\beta = \beta_0 \left(1-\exp(-\alpha t/T)\right)$} where $t$ denotes the current iteration, $T$ shows the total number of iterations, and $\alpha$ is a constant such that $\exp(-\alpha)\approx 0$. In Figure~\ref{fig:scheduled-momentum}, we compare the performance of MM, MM++, and MM++ with scheduled momentum (MM++: SM), and Block-Coordinate Minimization (BCM) \cite{erdogdu2018convergence} (which is similar to MM except for the coordinate selection procedure) with three different coordinate selection schemes: Uniform sampling (BCM: U), Importance sampling (BCM:I), and Greedy coordinate selection (BCM: G) for a MaxCut problem with $n=500$ nodes.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/scheduled_momentum.pdf}
    \caption{Comparison of Mixing Method (MM), Mixing Method++ with fixed momentum $\beta=0.8$ (MM++), Mixing Method++ with an increasing Scheduled Momentum from $0$ to $0.8$ (MM++: SM), and Block-Coordinate Minimization with Uniform sampling (BCM: U), Importance sampling (BCM: I), and Greedy coordinate selection (BCM:G), in terms of the objective cost per iteration.}
    \label{fig:scheduled-momentum}
\end{figure}

==> ICML20-AAAI21/Proofs/LemmaA1.tex <==
\clearpage
\subsection{Analogy of Lemma A1}
\begin{lemma}
\label{lemma:decreasing}
 Let $\hat{V}=M(V)$ for the Mixing method $M$ and  $g_i = \sum_{j< i} c_{i j} \hat{v}_j + \textcolor{red}{\beta v_i} + \sum_{j> i} c_{i j} v_j$
 $$
 f(V)-f(\hat{V})=2\sum_{i=1}^n(||g_i||-\beta)\cdot ||v_i-\hat{v}_i||^2
 $$
\end{lemma}
 \begin{proof*} The objective function $f$ w.r.t. variable $v_i$ while fixing all other variables $v_j$ is
 
 $$
 \langle C,V^\top V \rangle=\sum_{i=1}^n v_i^\top \left(\sum_j c_{ij}v_j \right) 
 $$
 Since only $v_i$ is changed during the $i$th coordinate-wise updating, the only part of objective value that will change is $2v_i^\top \left(\sum_{j<i}c_{ij}\hat{v}_j+\sum_{j>i}c_{ij}v_j\right)$. 
 Thus the updates of the Mixing method can be written as:
 
 $$\hat{v}_i=\frac{-g_i}{\|g_i\|_2}$$


Thus objective difference after updating $v_i$ to $\hat{v}_i$ is
\begin{align*}
2(g_i-\beta v_i)^\top \left(v_i-\hat{v}_i\right) &=  2\left(\|g_i\|_2-\beta \right) \left (1-v_i^\top\hat{v}_i \right) \\ &= 2\left(\|g_i\|_2-\beta \right) \|v_i-\hat{v}_i\|_2^2
\end{align*}
The result follows from  summing above equation over $i=1,...,n$
 \end{proof*}
 
 From Lemma \ref{lemma:decreasing} we can see that in order to guarantee strict decreasing of objective value, we have to assume that $\beta<||g_i||$. By assumption 3.1, $||g_i||\ge \delta$. Thus assume $\beta<\delta$ suffices. 
 

==> ICML20-AAAI21/Proofs/LemmaD2.tex <==
\clearpage
\subsection{Analogy of Lemma D.2}
\begin{lemma}
\label{lemma: lemma4}
Under the assumption 3.1 (see paper), there are constants $\gamma, \zeta$ such that
\begin{equation*}
    \left\lVert V - M(V)  \right \rVert \ge (\zeta - \gamma  \left\lVert y(V) - y(V^*) \right \rVert \, (f(V) - f^*).
\end{equation*}
 where $M: \mathbb{R}^{k \times n} \to \mathbb{R}^{k \times n} $, $y$ is the normalizer $\mathbb{R}^{k \times n} \to \mathbb{R}^n$, and $V^*$ is any optimum.
 
 More specifically, $\zeta =  \frac{\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}}{y^2_{max}}$ and $\gamma= \frac{2}{y^2_{min}} $
\end{lemma}

\begin{proof*} By \eqref{eq:matrix}, we can write $M(V)$ as $\,- V(L + \beta I) (L^\top +D_y)^{-1}$.  So 

\begin{equation*}
\begin{split}
 V - M(V ) =  V \big( I + (L + \beta I)(L^\top + D_y)^{-1} \big )  &= V(L ^ \top + D_y + L + \beta I) (L^\top + D_y) ^{-1},\\
 &= V(S + \beta I)(L^\top + D_y) ^{-1},
     \end{split}
\end{equation*}
where $S$ is $C + D_y$. 

Define $R$ as the matrix $(L^\top + D_y) ^{-1}$, and notice $S =  S^* + D_y - D_{y^*}$, then 
\begin{equation*}
\begin{split}
  \left\lVert  V - M(V )  \right \rVert_F ^2 & =  \left\lVert V(S + \beta I)R\, \right \rVert_F ^2\\
  &\ge \left\lVert V S R\, \right \rVert_F ^2 + 2 \text{ tr }(V^\top V S^* R R^\top (D_y-D_{y^*}+ \beta I))\\ 
  &\ge \sigma_{min}^2(R) \sigma_{min NZ}(S^*)\text{ tr }(V^\top V S^*) +  2 \text{ tr }(V^\top V S^* R R^\top (D_y-D_{y^*}))    + 2 \beta  \text{ tr }(V^\top V S^* R R^\top).
  \end{split}
\end{equation*}

Assuming $\text{ tr }(V^\top V S^* R R^\top (D_y-D_{y^*})) \ge  - \left\lVert y-y^* \right \rVert \sigma_{max}^2 (R) \text{ tr }(V^\top V S^*)$ and also that $\left\lVert y-y^* \right \rVert I + (D_y - D_{y^*}) \succeq 0$ still hold (see paper), we get the following chain of inequalities

\begin{equation*}
\begin{split}
  \left\lVert  V - M(V )  \right \rVert_F ^2 &\ge \sigma_{min}^2(R) \sigma_{min NZ}(S^*)\text{ tr }(V^\top V S^*)  - 2 \left\lVert y-y^* \right \rVert \sigma_{max}^2 (R) \text{ tr }(V^\top V S^*)  + 2 \beta \sigma_{min}^2(R)  \text{ tr }(V^\top V S^*)\\
  &=\bigg( \underbrace{\sigma_{min}^2(R)}_{1/y^2_{max}} \big(\,\sigma_{min NZ}(S^*)+ 2 \beta\, \big)- 2 \left\lVert y-y^* \right \rVert \underbrace{\sigma_{max}^2 (R)}_{1/y^2_{min}} \bigg) \underbrace{\text{ tr }(V^\top V S^*)}_{f(V)- f^*}\\
  &=\left( \frac{\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}}{y^2_{max}} - 2\frac{ \left\lVert y-y^* \right \rVert}{y^2_{min}}  \right) (f(V)- f^*).
  \end{split}
\end{equation*}
Since $y_{max}$ can be upper bounded by $\sum_{j}|c_{ij}|+\beta$ ($y_i=\|\sum_{j}c_{ij}V_j+\beta V_i\|$) and $y_{min}$ can be lower bounded by $\delta$ (Assumption \ref{assu:delta}), there exist $\zeta$ and $\gamma$ such that $\left\lVert V - M(V)  \right \rVert \ge (\zeta - \gamma  \left\lVert y(V) - y(V^*) \right \rVert \, (f(V) - f^*)$. Note that in the paper the bounds of $y_{min}$ and $y_{max}$ are not explicitly claimed. 
\end{proof*}
 Note that compared with Lemma D.2 in the paper, we have got a better lower bound of $\|V-M(V)\|_F^2$, given $\beta$ is positive.

==> ICML20-AAAI21/Proofs/LemmaD4.tex <==
\clearpage
\subsection{Analogy of Lemma D.4}
\begin{lemma}
\label{lemma: lemmad4}
Under the assumption 3.1 (see paper), let $M$ be the mixing method map. Then there is a constant $\tau > 0$ such that, for their normalizers $y^*  = y(V^*)$ and $y  = y(V)$, we get 

\begin{equation*}
    \left\lVert y- y^*  \right \rVert^2-3n\textcolor{red}{\beta}^ 2 \le \tau (f(V) - f^*).
\end{equation*}
More specifically, $\tau=3n(\rho_{max}(S^*)+\frac{(y_i^*)^2}{\delta})$
\end{lemma}

\begin{proof*}
Using the same notation as the authors, define $Z_i$ as the inner cyclic iterate before updating $v_i$ to $\hat v_i$, so that the only vector changed between $Z_i$ and $Z_{i+1}$ is $v_i$. So in each iteration we can thought in $Z_i$ as the matrix 
\begin{equation*}
    Z_i  = \begin{pmatrix}
    \vert  & & \vert & \vert & \vert && \vert \\
    \hat{v_1}   &\ldots & \hat{v}_{i-1} & v_i & v_{i+1} & \ldots & v_n\\
    \vert  & & \vert & \vert & \vert & & \vert
\end{pmatrix}.
\end{equation*}
That is, 
\begin{equation*}
    V = Z_1 \to Z_2 \to \ldots \to Z_n \to Z_{n+1} = M(V). 
\end{equation*}

As before let us define $S^* = C + D_{y^*}$, ($y_i = \|g_i\|$ and $D_{y^*}$ is $\text{diag}(y_1, \ldots, y_n)$, check matrix representation section). In each update we have the following result
\begin{equation*}
\begin{split}
    y_i \hat v_i &= - \left(\sum_{j< i} c_{i j} \hat{v}_j + \textcolor{red}{\beta v_i} + \sum_{j> i} c_{i j} v_j \right)\\
    & = -Z_i (c_i + \textcolor{red}{\beta} e_i).
\end{split}
\end{equation*}
where $c_i^\top$ is the $i$-th row of the matrix $C$. Then 

\begin{equation*}
    (y_i - y_i ^*)\hat{v_i} = -Z_i (c_i + \beta e_i) - y_i ^* \hat{v_i}. 
\end{equation*}
Since $ s_i ^* = c_i +  y_i ^*$, and also $Z_i y_i^*e_i  = v_i y_i^*$, we get 

\begin{equation}\label{eq:cycleupdate}
    (y_i - y_i ^*)\hat{v_i} = -Z_i (c_i + \beta e_i) - y_i ^* \hat{v_i} =  -Z_i s_i ^*+ y_i ^*(v_i-\hat{v_i})- \underbrace{Z_i e_i}_{v_i} \beta. 
\end{equation}
Notice that the terms $-Z_i s_i ^*$ and $(v_i-\hat{v_i})$ can be bounded by Lemma 3.12 and Assumption 3.1 (we assume that this property holds as in the original Mixing Method, but we have to check it),

\begin{equation}\label{eq:paperineq}
\begin{split}
    f(V)- f^{*}  &\ge f(Z_i) -f^{*} = \text{tr}(Z_i^\top Z_i S^*) \ge \frac{1}{\rho_{max}(S^*)} \|Z_i s_i^*\|^2,\\
     f(V)- f^{*}  & \ge f(Z_i) -f(Z_{i-1}) \ge \delta \|v_i - \hat{v}_i\|.
\end{split}
\end{equation}
 
It is easy to see that  $(y_i - y_i ^*)^2$ is $(y_i - y_i ^*)^2\hat{v_i}^\top \hat{v_i}$, i.e. it is the inner product of \eqref{eq:cycleupdate}. For brevity, define $a =-Z_i s_i$, $b = y_i ^*(v_i-\hat{v_i})$, and $c = -Z_i e_i \beta = -v_i \beta$. So 
\begin{equation*}
\begin{split}
    (a+b+c)^\top (a+b+c) &= a^\top a  +b^\top b+ c^\top c + \big(2 a^\top b + 2 c^\top a+ 2 b^\top c \big),\\
    &\le a^\top a  +b^\top b+ c^\top +  \big( 2 a^\top a  + 2 b^\top b+  2c^\top c \big)\\
    & = 3 ( a^\top a  +  b^\top b+  c^\top c).
\end{split}
\end{equation*}
for the last inequality, notice that for any vectors $u, v, w$ we have 

\begin{equation*}
    \begin{split}
   0 \le & (u-v)^\top (u-v) + (v- w)^\top(v- w) + (w-u)^\top (w-u) \\
     &= 2 u^\top u + 2 v ^\top v + 2 w ^\top w - 2 u ^\top v -2 v ^\top w - 2 w ^\top u,
    \end{split}
\end{equation*}
taking $u = a$, $v = b$ and $w = c$, the inequality follows. Thereby 

\begin{equation*}
(y_i - y_i ^*)^2 \le  3 \|Z_i s_i^*\|^ 2 + 3 (y_i^*)^2 \| v_i-\hat{v_i} \|^ 2  + 3\beta ^ 2.
\end{equation*}
So, using the previous result with the inequalities \eqref{eq:paperineq}, we get that $(y_i - y_i ^*)^2 $ is bounded by $f(V) - f^*$ and $\beta$ times some constant. Summing over $i = 1, \ldots, n$ we have the result for a constant $\tau > 0$.
\end{proof*}

==> ICML20-AAAI21/Proofs/MatrixRepresentation.tex <==
\clearpage
We define $C \in \mathbb{R}^{n\times n}$ the cost matrix of the problem and we assume that $C$ is symmetric

\begin{equation*}
    \text{min}_{V\in \mathbb{R}^{k \times n} } f(V) = \langle C, V^\top V \rangle \hspace{15 pt} \text{s.t.}\hspace{15 pt} \|v_i\| = 1 \hspace{15 pt} (i = 1, \ldots n).
\end{equation*}
i
Matrices $V$ and $\hat{V}$ refer to the current and the next iterate. 
Let us define:
\begin{equation*}
    g_i = \sum_{j< i} c_{i j} \hat{v}_j + \textcolor{red}{\beta v_i} + \sum_{j> i} c_{i j} v_j.
\end{equation*}

For all $i \in \{1, \ldots n\}$ in each cycle, the iteration uses the most recently available information of $\hat{v}_i$. For example $\hat{v}_1$ is used in the calculation of $\hat{v}_2$ and so on. Then if we put the elements of $\hat{V}$ in the left and the one of $V$ in the right, we obtain
\begin{algorithmic}
\FOR {$1:n$}
    \STATE \begin{equation}\label{eq:matrix}
        \sum_{j< i} c_{i j} \hat{v}_j+ \|g_i\| \hat{v}_i =  - \left( \textcolor{red}{\beta v_i} + \sum_{j> i} c_{i j}  v_j\right).
    \end{equation}
\ENDFOR
\end{algorithmic}

The transition from $V$ to $\hat{V}$ can be succinctly expressed in terms of $C$. Let $L$ be the strictly lower triangular matrix
\begin{equation*}
 L_{ij} = 
    \begin{cases}
    c_{i j}& \hspace{10pt} \text{for $i > j$}\\
    0& \hspace{10pt}\text{for $i < j$}.
    \end{cases}
\end{equation*}

By symmetry, the associated strictly upper triangular matrix is $L^\top$. Let $D_y = \text{diag}(\|g_1\|, \ldots, \|g_n\|)$. Let $M: \mathbb{R}^{k\times n} \to  \mathbb{R}^{k\times n}$ be the mapping of the mixing method with acceleration, that is M(V) is
\begin{equation*}
    M(V) = \begin{bmatrix} \hat{v}_1, \ldots, \hat{v}_n \end{bmatrix}.
\end{equation*}

Using \eqref{eq:matrix}, $L$ and $D_y$ we get

\begin{equation}\label{eq:matrixform}
    (L+D_y)\,M(V)^\top = - (L^\top + \textcolor{red}{\beta} I)\, V^\top
\end{equation}
By assumption $\|g_i\| > 0$, $L+D_y$ is invertible and hence, $M(V)^\top = - (L+D_y)^{-1}(L^\top + \beta I)\, V^\top$.

==> ICML20-AAAI21/Proofs/Theorem3.5.tex <==
\clearpage
\subsection{Analogy of Theorem 3.5 (linear convergence)}

By Lemma D.2 (analogy), there are constants $\zeta$ and $\gamma$ such that

 $$\left\lVert V - M(V)  \right \rVert \ge (\zeta - \gamma  \left\lVert y(V) - y(V^*) \right \rVert \, (f(V) - f^*).$$
 
 For some $\kappa>0$, we want to pick a neighborhood close enough to the optimum where $f(V)-f^*$ is sufficiently small so that $\zeta-\gamma\|y-y^*\|\ge \kappa >0$, in other words, $\|y-y^*\|\le \frac{\zeta-\kappa}{\gamma}$.
  Note that every $\kappa\le \zeta$ is feasible. We have
  $$\|V-M(V)\|^2\ge \kappa (f(V)-f^*)$$.
  Further, the above inequality holds for all subsequent iterates, because $f(V)-f^*$ is strictly decreasing under the assumption $\beta< \delta$, thus still sufficiently small so that $\zeta-\gamma\|y-y^*\|\ge \kappa\ge 0$ holds. Together with Lemma A.1, there is another constant $2(\delta-\beta)>0$ such that $f(V)-f(M(V))\ge 2(\delta-\beta)\|V-M(V)\|^2$, and thus
  $$f(V)-f(M(V))\ge 2(\delta-\beta)\kappa(f(V)-f^*)\Longrightarrow  f(M(V))-f^*\le (1-2(\delta-\beta)\kappa)(f(V)-f^*)$$
 
 Thus the accelerated version of Mixing Method has linear convergence. The linear convergence rate is $1-2(\delta-\beta)\kappa$.
 
 Next we want to decide the order of $\beta$. Note that $\kappa\le \zeta$. By Lemma D.4 (analogy), it is suffices to have 
 $$3n\beta^2+\tau(f(V)-f^*)\le
( \frac{\zeta-\kappa}{\gamma})^2$$
 
 Thus the region where linear convergence happens is 
 $$f(V)-f^*\le \frac{1}{\tau}((\frac{\zeta-\kappa}{\gamma})^2-3n\beta ^2)$$
 
 Since the region should have size large than 0, we have 
 $$\frac{1}{\tau}((\frac{\zeta-\kappa}{\gamma})^2-3n\beta ^2)\ge 0$$
 
 Since $\gamma = \frac{2}{y^2_{min}}$ and $\zeta= \frac{\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}}{y^2_{max}}$

$$\frac{y_{min}^4}{4}( \frac{\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}}{y^2_{max}})-\kappa)^2\ge 3n\beta^2$$

$$\frac{y_{min}^2}{2}( \frac{\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}}{y^2_{max}})-\kappa)\ge \sqrt{(3n)}\beta$$

$$\beta\le \frac{\sigma_{min NZ}(S^*)-y_{max}^2\kappa}{2\sqrt{3}(\frac{y_{max}}{y_{min}})^2\sqrt{n}-2}\le \frac{\sigma_{min NZ}(S^*)}{2\sqrt{3}(\frac{y_{max}}{y_{min}})^2\sqrt{n}-2}=O(\frac{1}{\sqrt{n}})$$.

\textcolor{blue}{Zhiwei: I found that the bound of $\sigma_{min NZ}$ and $y_{max}$ will change after adding $\beta$. Thus the comparison in the following is not correct.}

For a comparison between Accelerated Mixing Method and Mixing Method, see Table \ref{comparison}.
\begin{table}[h!]
\centering
\resizebox{1.2\textwidth}{!}{
\begin{tabular}{|l|l|l|ll}
\cline{1-3}
                        & Mixing & Accelerated Mixing &  &  \\ \cline{1-3}
Linear convergence Rate & $(1-2\kappa\delta)$    & $(1-2\kappa(\delta-\beta))$              \\ \cline{1-3}
Linear Conv. Region $(f(V)-f^*)$                  &$\frac{3}{2\tau \gamma^2}{(\zeta-\frac{2\beta}{y^2_{max}}-\kappa)^2}$     &     $\frac{1}{\tau \gamma^2}((\zeta-\kappa)^2-3n\gamma^2\beta^2)$           \\ \cline{1-3}
Maximum $\kappa$& $\zeta- \frac{2\beta}{y^2_{max}}$   & $\zeta$              \\ \cline{1-3}
\end{tabular}}
\caption{Comparison between Acc. Mixing and Mixing}
\label{comparison}
\end{table}

In which case will we get a better linear convergence rate? Let $\kappa_M=\zeta- \frac{2\beta}{y^2_{max}}$ be the maximum $\kappa$ of Mixing Method and $\kappa_{AM}=\zeta$ be the maximum $\kappa$ of accelerated Mixing Method. We need to have $(1-\kappa_M\delta)>(1-\kappa_{AM}(\delta-\beta))$.

$$(1-\zeta\delta+ \frac{2\beta}{y^2_{max}}\delta)>1-\zeta(\delta-\beta)$$

$$\frac{2\beta}{y^2_{max}}\delta>\zeta\beta$$


Recall that $\zeta= \frac{\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}}{y^2_{max}}$, we need


$$\frac{2\beta}{y^2_{max}}\delta>\frac{\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}}{y^2_{max}}\beta$$

$$2\delta>\sigma_{min NZ}(S^*)+ 2 \textcolor{red}{\beta}$$

Recall that $\beta<\delta$. Thus if we assume $\sigma_{min NZ}(S^*)<2(\delta-\beta)$, we can get a better convergence rate by having a positive $\beta$.
\begin{remark}
The problem with our previous analysis is, $y_{min}$, $y_{max}$, $\delta$ and $\sigma_{minNZ(S^*)}$ are not real "constants", but functions of $\beta$. If we don't consider this into account, we might not be able to capture the acceleration in theory. 
To demonstrate this fact, I did a simple experiment which watches $y_{min}$ and $y_{max}$ (See Table \ref{table:g27}, \ref{table:g62}).

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
$\beta$ & $y_{max}$ & upper bound of $y_{max} $ in theory & $y_{min}$ \\ \hline
-0.3    & 14.83     & 20.3                     & 2.78      \\ \hline
0       & 14.53     & 20                       & 2.72      \\ \hline
0.3     & 14.23     & 20.3                     & 2.69      \\ \hline
0.6     & 13.92     & 20.6                     & 2.67      \\ \hline
0.9     & 13.62     & 20.9                     & 2.37      \\ \hline
1.2     & 13.31     & 21.2                     & 2.07      \\ \hline
1.5     & 12.99     & 21.5                     & 1.77      \\ \hline
1.8     & 12.69     & 21.8                     & 1.47      \\ \hline
2.1     & 12.37     & 22.1                     & 1.20      \\ \hline
\end{tabular}
\caption{G27}
\label{table:g27}
\end{table}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
$\beta$ & $y_{max}$ & upper bound of $y_{max}$ in theory & $y_{min}$ \\ \hline
-0.3    & 4.28      & 4.3                      & 1.56      \\ \hline
0       & 3.98      & 4                        & 1.45      \\ \hline
0.3     & 3.68      & 4.3                      & 1.31      \\ \hline
0.6     & 3.38      & 4.6                      & 1.01      \\ \hline
0.9     & 3.08      & 4.9                      & 0.77      \\ \hline
\end{tabular}
\caption{G62}
\label{table:g62}
\end{table}

From the table we see that as $\beta$ increases, $y_max$ decreases with almost the same amount of $\beta$'s increment. $y_min$ also decreases but the pattern is not obvious.

How do we get the upper bound of $y_{max}$ in theory?

$$y_i=\|g_i\|= \|\sum_{j< i} c_{i j} \hat{v}_j + \textcolor{red}{\beta v_i} + \sum_{j> i} c_{i j} v_j\|\le \sum_j{|c_{ij}|}+\beta$$

Note that the inequality uses all $v_j$ and $\hat{v_j}$ are unit.

However what we didn't capture is that as the algorithm converges, $\beta v_i$ has the direction almost opposite with $ \sum_{j< i} c_{i j} \hat{v}_j  + \sum_{j> i} c_{i j} v_j$, which is the reason of adding beta decreases $y_{max}$ instead of increasing in theory. In my opinion, we need some theory to characterize this fact.  If we can show that $y_{max}$ decreases after adding $\beta$, we are one step closer to show where acceleration hides.

Note that we also want to characterize $\delta$ $(y_{min})$ and $\sigma_{minNZ}(S^*)$ but currently I have no idea yet.
\end{remark}

==> ICML20-AAAI21/Proofs_Algorithm_2/LemmaA1.tex <==
\subsection*{Proof of Lemma \ref{lemma:decreasing}}

\begin{proof}
Let $\beta$ be in $[0, 1]$.  When fixing all the others variables, $f$ with respect to $v_i$ is given by
\begin{equation*}
     \langle C,V^\top V \rangle= 2 v_i^\top \left(\sum_j c_{ij}v_j \right)+ \text{constant}.
\end{equation*}

Since only $v_i$ is changed, during the $i$th coordinate-wise updating, the only part of the objective that will change is $2v_i^\top g_i$. That is,
\begin{equation*}
 f(Z_i(V))-f(Z_{i+1}(V)) = 2g_i^\top \left(v_i-\hat{v}_i\right). 
\end{equation*}

The updating rule of algorithm \ref{algo:accelerated_mixing} is given by the recursion \eqref{eq:recursion}, so using this into the above equation yields
\begin{equation*}
\begin{split}
   f(Z_i(V))-f(Z_{i+1}(V)) &= \frac{2y_i\,(w_i- \beta)}{1+\beta}(1-v_i^\top \hat{v}_i),\\
    &= \frac{y_i\, (w_i- \beta)}{1+\beta}\|v_i - \hat{v}_i\|_2^2.
\end{split}
\end{equation*}

From observation \ref{observation0}, we have  $w_i-\beta \ge 1-\beta$. Thus,
\begin{equation*}
\begin{split}
    f(Z_i(V))-f(Z_{i+1}(V)) \ge y_i\, \frac{1- \beta}{1+\beta}\|v_i - \hat{v}_i\|_2^2.
\end{split}
\end{equation*}
Adding over all the $i$, leads us to the desired conclusion 
\begin{equation*}
\begin{split}
    f(V)-f(\hat{V}) &= \sum_{i= 1}^n\,f(Z_i(V))-f(Z_{i+1}(V)) \\
    &\ge \frac{1-\beta}{1+\beta}\sum_{i= 1}^n y_i\,\|v_i - \hat{v}_i\|_2^2.
    \end{split}
\end{equation*}
\end{proof}

==> ICML20-AAAI21/Proofs_Algorithm_2/LemmaD2.tex <==
\subsection*{Proof of Lemma \ref{lemma: lemmad2}}

\begin{proof}
 
By~\eqref{eq:matrixformA2}, we have
\begin{align*}
    \hat{V} =\,- V\left(\left(1+\beta\right)L + \beta D_y\right) \left(\left(1+\beta\right)L^\top +D_w D_y\right)^{-1}.
\end{align*}
% Thus,  can be inferred that:
This leads to
\begin{align*}
\begin{split}
 V -\hat{V}
 =& V(\left(1+\beta\right)C + D_wD_y + \beta D_y)\\
 &(\left(1+\beta\right)L^\top + D_wD_y) ^{-1}\\
 =& V S \underbrace{(\left(1+\beta\right)L^\top + D_wD_y) ^{-1}}_{R},
     \end{split}
\end{align*}

% By definition of \mbox{$\Delta\triangleq (D_wD_y+\beta D_y)- (D_{w^*}D_{y^*}+\beta D_{y^*})$} and the fact that \mbox{$S =  S^*+\Delta$} in the previous equation we get
Using the definition \mbox{$\Delta\triangleq (D_wD_y+\beta D_y)- (D_{w^*}D_{y^*}+\beta D_{y^*})$}, and the fact that \mbox{$S =  S^*+\Delta$} in the previous equation, we get
%
\begin{equation}\label{eq:inequalityAlg2}
    \begin{split}
        \|V-\hat{V}\|_F^2 
        &\ge  \|VS^*R\|_F^2 + 2 \text{tr}\big(V^\top VS^* R R^\top \Delta\big).
    \end{split}
\end{equation}
%
We claim that $$\|(w+\beta \mathds{1})\odot y- (w^*+\beta \mathds{1})\odot  y^*\|_2 I_n + \Delta	\succeq 0.$$
To see this, first notice \mbox{$D_wD_y+ \beta D_y = D_{(w+\beta \mathds{1})\odot y}$}. Thus,
$$ \Delta = D_{(w+\beta \mathds{1})\odot y}- D_{(w^*+\beta \mathds{1})\odot y^*}.$$
%
Besides, 
$$\|(w+\beta \mathds{1})\odot y- (w^*+\beta \mathds{1})\odot  y^*\|_2 = \| \Delta \|_F.$$
%
So the claim follows since $\beta \ge 0$ and termwise 
\begin{equation*}
    \begin{split}
        \| \Delta \|_F+ \Delta_i \ge |\Delta_i |+ \Delta_i \ge 0. 
    \end{split}
\end{equation*}
%
Now, for the first part in \eqref{eq:inequalityAlg2}, we get 
\begin{equation*}
\begin{split}
    \|VS^*R\|_F^2 &= \text{tr}(\underbrace{{S^*}^\top}_{\succeq 0} \underbrace{V^\top V}_{\succeq 0} \underbrace{S^*}_{\succeq 0} \underbrace{R R^\top}_{\succeq 0}) \\
    &\ge \sigma_{\min}^2(R) \sigma_{\texttt{nnz}}(S^*) \text{tr}(V^TV S^*).
\end{split}
\end{equation*}
%
For the second in \eqref{eq:inequalityAlg2}, we get
\begin{equation*}
    \begin{split}  \text{tr}\big(V^\top VS^* R R^\top \Delta\big) &\ge -\|\Delta\|_F\tr\big(V^\top VS^* R R^\top\big)\\
    &\ge-\|\Delta\|_F\,\sigma_{\max}^2(R)\text{tr}\big(V^\top VS^*\big),
    \end{split}
\end{equation*}
this last inequality is given by our previous claim, the fact that $S^* \succeq 0$ (observation \ref{PSD}) and 
\begin{equation*}
    \begin{split}
        \tr(V^\top VS^*RR^\top) &=\tr(V^\top VS^*\underbrace{UD^2U^\top}_{RR^\top}) \\ &=\tr(V^\top VS^*D^2)\\
        &\le \sigma^2_{\max}(R) \, \tr(V^\top VS^*).
    \end{split}
\end{equation*}
%
Using the lower bounds in \eqref{eq:inequalityAlg2} gives us
\begin{equation*}
    \begin{split}
        \|V&-\hat{V}\|_F^2\\ 
        &\ge \big(\sigma_{\min}^2(R) \sigma_{\texttt{nnz}}(S^*) -2\|\Delta\|_F\sigma_{\max}^2(R)\big)\text{tr}\big(V^\top VS^*\big).
    \end{split}
\end{equation*}
To conclude, the term 
\begin{equation*}
    \begin{split}
      \tr(V^\top VS^*) &= \tr(V^\top VC)-\tr(-V^\top V D_{y^*} )\\
      &= f(V) - \tr(-V^\top V D_{y^*})\\
      &\stackrel{i)}{=} f(V) - \sum\limits_{i} - \left (\underbrace{\langle v_i, v_i \rangle}_{=1} \cdot y^*_i \right )\\
      &= f(V) - (-\langle \mathds{1}, y^* \rangle )\\   
      &\stackrel{ii)}{\geq} f(V) - f^*.
    \end{split}
\end{equation*}
where $i)$ follows from the fact that $D_{y^*}$ is diagonal. 
To understand $ii)$, consider the dual to the diagonally constrained SDP problem \eqref{eq:continuous_form} (i.e., see Lemma 3.12 of \cite{wang2017mixing} for more details).

\begin{align}
    \max\limits_{y} -\langle \mathds{1}, y \rangle, ~\text{such that } C + D_y \succeq 0
    \label{dual_sdp}
\end{align}
%
We know that \mbox{$C + D_{y^*} = \frac{S^*}{1+\beta} \succeq 0$} from Observation \ref{PSD}.
Therefore, $y^*$ is a feasible solution to the dual problem \eqref{dual_sdp}, revealing that \mbox{$f^* \geq - \langle \mathds{1}, y^* \rangle$}.
%
This fact allows us to derive the inequality given by $ii)$.
Then, if we define \mbox{$\zeta = \sigma^2_{\min} (R)\sigma_{nnz} (S^*)$} and \mbox{$\gamma = 2\sigma^2_{\max} (R)$} with \mbox{$\sigma_{\min}(R) = 1/(w\odot y)_{\max}$} and \mbox{$\sigma_{\max}(R) = 1/(w\odot y)_{\min}$}, we arrive at the final result.
%
\begin{align*}
    \|V - \hat{V}\|^2_F \geq \left(\zeta - \gamma \|\Delta\|_F\right)(f(V) - f^\star)
\end{align*}
%
It should be noted that both $\zeta$ and $\gamma$ are strictly positive constants because $R$ is defined as an invertible matrix and, therefore, has all non-zero eigenvalues.
\end{proof}

==> ICML20-AAAI21/Proofs_Algorithm_2/MatrixRepresentation.tex <==
\subsection*{Matrix Representation}
The transition from the state $v_i$ to $\hat{v}_i$ is expressed in the relation \eqref{eq:recursion}, then for any $i \in [n]$ in each inner cycle we have, 
\begin{align}\label{eq:matrixA2}
\begin{split}
   \left(1+\beta\right)\sum_{j< i} c_{i j} \hat{v}_j + w_i y_i \hat{v}_i =-\left(1+\beta\right)\sum_{j> i} c_{i j}  v_j - \beta y_i v_i.
\end{split}
\end{align}
Let $L$ be the strictly lower triangular matrix of $C$ so \eqref{eq:matrixA2} leads us to the representation 

\begin{align}\label{eq:matrixformA2}
    \left(\left(1+\beta\right)L+ D_w D_y\right)\, \hat{V}^\top = - \left(\left(1+\beta\right)L^\top + \beta D_y\right)\, V^\top.
\end{align}

==> ICML20-AAAI21/Proofs_Algorithm_2/Theorem3.2.tex <==
\begin{theorem*}
Let $V^\ell = Z_{n+1}^\ell(V)$, see definition \eqref{eq: Z}, for all $\ell\in \mathbb{N}$; i.e., the collection of points generated by \texttt{Mixing Method++} after finishing the inner loop. Then, under the assumption \ref{assu:delta}, $\{V^\ell\}_\ell$ converges to a limit point $\bar{V}$ and the riemannian gradient at $\bar{V}$ is zero (\texttt{Mixing Method++} converges to a first-order critical point).  
\end{theorem*}


\textcolor{red}{xx Lyle: we need to fix this part xx}
\begin{proof}
For $\beta$ in $[0, 1/2)$ we know by lemma \ref{lemma:decreasing} that the objective function is decreasing. Besides, $(S^{k-1})^n$ is compact, indeed limit point compact, so there exists a limit point $\bar{V}$ such that $f(\bar{V}) = \lim_k f(V^k)$ by continuity of $f$. It is clear that $\bar V$ is a fixed point in relation \eqref{eq:matrixformA2}, so

\begin{equation}\label{eq:equilibrium}
   \bar{V} C = - \bar{V} D_{(\bar{w}+ \beta \mathds{1}) \odot \bar{y}} .
\end{equation}

Since the constraint set is a product of spheres, its corresponding tangent space (henceforth denoted by the letter $\mathrm{T}$) at the point $\bar{V}$ is given by the product of tangent spaces of $S^{k-1}$; namely

\begin{equation}\label{eq:ManProd}
    \mathrm{T}_{\bar{V}} \left(S^{k-1}\right )^n = \prod_{j=1}^n \mathrm{T}_{\bar{v_j}}\, \left(S^{k-1}\right),
\end{equation}
where $\bar{v}_j$ is the $j$th column of $\bar V$. 

The above result gives us a way to characterize the tangent space. To this end, it is actually enough to work with the tangent space of $S^{k-1}$. 

By definition, for any $v_j$, the vector $\dot{v}_j\in \mathbb{R}^k$ is in the tangent space of $S^{k-1}$ if and only if there exists a curve $\varphi: I \to S^{k-1}$ such that $\varphi(0) = v_j $ and $\dot{\varphi}(0) = \dot{v}_j$, where $\dot{\varphi}$ is the derivative of $\varphi$. Then $\varphi(t) \in S^{k-1}$ if satisfies $ \langle \varphi(t), \varphi(t) \rangle  = 1$ for all $t\in I$. Differentiating on both sides leads us to $0 = \langle  \dot{\varphi}(t), \varphi(t) \rangle  + \langle \varphi(t), \dot{\varphi}(t) \rangle$. Evaluating at $t = 0$, we get 
\begin{equation*}
     2 \langle  \dot{v}_j,  v_j \rangle  = 0,
\end{equation*}
thus $\{\dot{v}_j \in \mathbb{R}^k : \langle  \dot{v}_j,  v_j \rangle  = 0 \} \subseteq \mathrm{T}_{v_j} S^{k-1}$, since both subspaces are of the same dimension, $\{\dot{v}_j \in \mathbb{R}^k : \langle  \dot{v}_j,  v_j \rangle = 0  \}  = \mathrm{T}_{v_j} S^{k-1}$.

Now by \eqref{eq:ManProd} and the previous analysis, we finally arrive to the characterization of the tangent space; namely 
\begin{equation*}
    \mathrm{T}_{\bar{V}} \left(S^{k-1}\right)^n = \left\{ \dot{\bar{V}} \in \mathbb{R}^{k\times n} :  \langle  \dot{\bar{v}}_j,  \bar{v}_j \rangle = 0 \hspace{5 pt} \forall j \in [n]\, \right\},
\end{equation*}
and $\dot{\bar{v}}_j$ ($v_j$) corresponds to the $j$th column of $\dot{\bar{V}}$ ($\bar{V}$), respectively.

Let $\mathrm{P}^\perp: \mathbb{R}^{k\times n}  \to  \mathrm{T}_{\bar{V}} \left(S^{k-1}\right)^n$ be the projector operator from the euclidean space to the tangent space at $\bar{V}$, defined for any $W \in \mathbb{R}^{k\times n}$ as follows,
\begin{equation*}
    W  \xrightarrow{ \mathrm{P}^\perp}  \begin{pmatrix}

   w_1 -   \langle  \bar{v}_1,  w_1 \rangle \bar{v}_1     & \ldots  & w_n -\langle  \bar{v}_n,  w_n \rangle \bar{v}_n 
\end{pmatrix}.
\end{equation*}

Let the riemannian gradient of $f$ denoted by $\mathrm{grad}f(\cdot)$, and the gradient of $f$ defined in the entire euclidean domain as $\nabla f (\cdot)$, so using tools from matrix manifold the riemannian gradient is given by 

$$\mathrm{grad}f(\bar{V}) = \mathrm{P}^\perp (\nabla f(\bar{V})).$$  
It is easy to see that $\nabla f(\bar{V}) = 2 \bar{V}C$, and by relation \eqref{eq:equilibrium}, this yields us to the equivalent version $\nabla f(\bar{V}) =  -2 \bar{V} D_{(\bar{w}+ \beta \mathds{1}) \odot \bar{y}}$. 

To conclude, let us fix a coordinate, say $j\in [n]$, so $\left(\nabla f(\bar{V}) \right)_j = -2(w_j y_j + \beta y_j  ) \bar{v}_j$ and by definition of the projection map we get 
\begin{equation*}
\begin{split}
     \left( \mathrm{P}^\perp(\nabla f(\bar{V}) \right) _j  =  2(w_j y_j + \beta y_j  )  (- \bar{v}_j  +\bar{v}_j) = 0.
\end{split}
\end{equation*}
So for all the coordinates $\left( \mathrm{P}^\perp(\nabla f(\bar{V}) \right) _j = 0$, and thus $\mathrm{P}^\perp(\nabla f(\bar{V}) = \mathrm{grad}f(\bar{V})  = 0$.
\end{proof}

==> ICML20-AAAI21/Proofs_Algorithm_2/Theorem3.5.tex <==
\subsection*{Proof of Theorem \ref{theorem: linearconvergence}}
\begin{proof}

Based on Lemma \ref{lemma: lemmad4}, a neighborhood can be selected around the optimum such that the value of $f(V) - f^\star$ is sufficiently small. 
In particular, we define this neighborhood through the selection of a positive constant $\kappa$ such that the following inequality holds, where $\tau$ is defined in Lemma \ref{lemma: lemmad4}.

\begin{align}
    \left ( \frac{\zeta - \kappa}{\gamma}\right )^2 \geq \tau \left ( f(V) - f^\star \right) \label{neighborhood_exp}
\end{align}

Within this expression, $\zeta$ and $\gamma$ are both defined in Lemma \ref{lemma: lemmad2}.
Because $\zeta$ and $\gamma$ are both strictly positive (i.e., see Lemma \ref{lemma: lemmad2}), $\left ( \frac{\zeta - \kappa}{\gamma} \right )$ is known to be strictly positive so long as $\kappa \in [0, \zeta)$.
Therefore, there always exists a value of $\kappa$ such that \eqref{neighborhood_exp} will be true within a sufficiently small neighborhood around the optimum. 
From here, we combine \eqref{neighborhood_exp} with the inequality from Lemma \ref{lemma: lemmad4} to yield the following.

\begin{equation*}
    \left(\frac{\zeta - \kappa}{\gamma} \right)^ 2\ge \tau (f(V)- f^*) \ge \|\Delta\|_F^ 2,
\end{equation*}
Then, because $\left ( \frac{\zeta - \kappa}{\gamma} \right )$ is strictly positive, we can manipulate the above expression to yield the following. 

\begin{equation}
    \zeta - \gamma\|\Delta\|_F  \ge \kappa. \label{kappa_bound}
\end{equation}

The above inequality holds for all successive iterations of Algorithm \ref{algo:accelerated_mixing}.

Then, based on the combination of Lemma \ref{lemma:decreasing} and assumption \ref{assu:delta}, $f(V)- f(\hat{V}) \ge  \delta\frac{1-\beta}{1+\beta}\|V - \hat{V}\|_F^ 2$, and thus 
\begin{equation*}
\begin{split}
    f(V)- f(\hat{V}) &\ge  \delta \frac{1-\beta}{1+\beta}\|V - \hat{V}\|_F^ 2\\
                  &\stackrel{i)}{\ge}  \delta\frac{1-\beta}{1+\beta} \kappa (f(V)-f^*)
\end{split}
\end{equation*}
where $i)$ is derived by combining \eqref{kappa_bound} and Lemma \ref{lemma: lemmad2}.
This expression in turn implies the following.
\begin{equation*}
    \left(1- \delta \kappa \frac{1-\beta}{1+\beta}\right)(f(V)-f^*) \ge f(\hat{V})-f^*.
\end{equation*}
thus giving us the desired linear convergence.
\end{proof}

==> ICML20-AAAI21/Proofs_Algorithm_2/lemmaD4.tex <==
\subsection*{Proof of Lemma \ref{lemma: lemmad4}}

\begin{proof}
Recall that $\Delta_i = (w_i + \beta) y_i - (w_i^\star + \beta) y_i^\star$.
We can unroll the value of $\Delta_i \hat{v}_i$ into the following expression.
\begin{align}\label{eq:difference}
        \big((w_iy_i -w_i^*y_i^*)+ \beta(y_i-y_i^*)\big)\, \hat{v_i}
\end{align}
Then, we derive the following equality from \eqref{eq:recursion}.
\begin{equation}
\begin{split}
    w_i y_i\hat{v_i} &= -\left(1+\beta\right)g_i - \beta y_i v_i \\
    &= -\left(1+\beta\right)Z_i c_i - \beta y_i v_i \label{eq:recursion_unrolled}
\end{split}
\end{equation}
where we denote \mbox{$Z_i = Z_i(V)$} for brevity and $c_i$ as the $i$th column of $C$.
We denote \mbox{$s_i^*  = \left(1+\beta\right)c_i +w_i^*y_i ^* e_i + \beta y_i ^* e_i$}.
By adding~\eqref{eq:difference} to both sides of~\eqref{eq:recursion_unrolled}, we arrive at the following, expanded version of the update rule in \eqref{eq:recursion}.
\begin{equation}\label{eq:eqSubs}
    \begin{split}
        & w_iy_i \hat{v_i} -w_i^*y_i^* \hat{v_i}+ \beta y_i \hat{v_i} - \beta y_i^*\hat{v_i}\\
        &= -\left(1+\beta\right)Z_i c_i - \beta y_i v_i -w_i^*y_i^* \hat{v_i}+ \beta y_i \hat{v_i} - \beta y_i^*\hat{v_i}\\
        &\stackrel{i)}{=} -Z_i s_i^ *+ \big(w_i^*y_i^* - \beta (y_i -y_i^ *) \big) (v_i - \hat{v_i}).
    \end{split}
\end{equation}
where $i)$ follows from the definition of $s_i^\star$ and the fact that $Z_i e_i = v_i$.
By combining Assumption~\ref{assu:delta} and Lemma~\ref{lemma:decreasing}, it is known that
\begin{equation}\label{eq:ineq1}
    f(V)- f^ * \ge   \frac{1-\beta}{1+\beta}\,\delta \, \|v_i - \hat{v_i} \|_2^2.
\end{equation}
Besides,
\begin{equation}\label{eq:ineq2}
\begin{split}
    f(V)- f^*&\ge f(Z_i)- f^*\\
    &= \tr(Z_i^\top Z_i S^*)\\&\ge \sigma^{-1}_{\max}(S^*)\|Z_i S^*\|_F^2\\
    &\ge \sigma^{-1}_{\max}(S^*)\|Z_i s_i^*\|_2^2 
\end{split}
\end{equation}

Therefore, based on \eqref{eq:ineq1} and \eqref{eq:ineq2}, it is known that \mbox{$\|Z_i s_i^\star\|_2^2$} and \mbox{$\|v_i - \hat{v}_i\|^2_2$} are both upper bounded by a positive factor of \mbox{$f(V) - f^\star$}.
We take the inner product of \eqref{eq:difference} with itself to yield the following.
\begin{align*}
    \Delta_i^2 &\stackrel{i)}{=} \big((w_iy_i -w_i^*y_i^*)+ \beta(y_i-y_i^*)\big)^2\\
    &\stackrel{ii)}{\le}2 \|Z_i s_i^ *\|^ 2  + 2 (y^*_i-\beta y_i)^2 \|v_i - \hat{v_i}\|^2 \\
    &=2 \|Z_i s_i^ *\|^ 2  + 2 ({y^*_i}^2-2\beta y_i^*y_i+ {y_i}^ 2)\, \|v_i - \hat{v_i}\|^2\\
\end{align*}

where $i)$ follows from the fact that $\hat{v}_i$ is a unit vector and $ii)$ follows from combining observation \ref{observation} with \eqref{eq:eqSubs}. 
From here, one can notice that $$\|(w+\beta \mathds{1})\odot y- (w^*+\beta \mathds{1})\odot  y^*\|_2^2 = \|\Delta\|_F^2 = \sum\limits_{i=1}^{n} \Delta_i^2$$.
We combine this expression with the upper bounds for \mbox{$\|Z_i s_i^\star\|^2_2$} and \mbox{$\|v_i - \hat{v}_i\|^2_2$} derived in \eqref{eq:ineq1} and \eqref{eq:ineq2} to arrive at the final result, where $\tau$ is defined as some positive constant.

\begin{align*}
\|(w+\beta \mathds{1})\odot y- (w^*+\beta \mathds{1})\odot  y^*\|_2^2 \le \tau (f(V) - f^*)
\end{align*}

\end{proof}

==> ICML20-AAAI21/Proofs_Algorithm_2/notation.tex <==
%\subsection{Notation}\label{notation} 
%Let us first define our notation we shall use throughout the paper. In general, we follow \cite{wang2017mixing}, except when it may be a reason for confusion.

\noindent
\textbf{Notation.} We use $\mathbb{S}^n$ to denote the cone of positive semi-definite matrices (PSD). 
For clarity, the $(k-1)$-dimensional sphere shall be denoted by $\text{Sph}^{k-1}$. 
For any $v\in \mathbb{R}^n$ and $M\in \mathbb{R}^{n\times m}$, we define $\|v\|_2 $ and $\|M\|_F $ as the norm induced by its corresponding inner product; namely, $\|\xi \|_{*} = \langle \xi, \xi \rangle^{1/2}_{**}$, for $\xi \in \{\mathbb{R}^n, \mathbb{R}^{n\times k}\}$, $*\in \{2, F\}$ and $**\in \{\mathbb{R}^n, \mathbb{S}^n\}$.

For a matrix $V \in \mathbb{R}^{k \times n}$, we interchangeably denote its $i$-th column as $V_{:, i}$ or $v_i$. 

For any $a$ in $\mathbb{R}^n$, we define $D_a$ as the matrix $\text{diag}(a)$; namely, $(D_a)_{ii} = a_i$. 
The vector $\mathds{1}$ represents the vector of only $1$'s, and its dimension is apparent from the context. 
The matrix $C$ corresponds to the cost matrix of the optimization problem \eqref{eq:continuous_form}. We shall assume $C\in \mathbb{S}^n$, if this were not so, notice that $C$ in \eqref{eq:discrete_form} can always be replaced by a matrix $C'\in \mathbb{S}^n$ such that $x^\dagger C x = x^\dagger C' x$. 


\noindent
\textbf{Low-rankness and SDPs.}
Focusing on \eqref{eq:continuous_form}, the set of linear constraints are far less than the number of variables in $X$. 
This constitutes such SDPs as \emph{weakly constrained}; weakly constrained SDPs provably have low-rank solutions because of the geometry of the set of PSD matrices, as noted below:
\begin{lemma}\cite{barvinok1995problems, pataki1998rank}
The SDP problem formulation in \eqref{eq:continuous_form} has a solution with rank $k$, where $k = \left \lceil \sqrt{2n} \right \rceil$.\footnote{Under the assumption that the search space in formulation  \eqref{eq:continuous_form} is compact.}
\end{lemma}
%By the previous work of \cite{pataki1998rank, barvinok1995problems} and the fact that , \eqref{eq:continuous_form} admits a lower-rank global optimum. 
One can exploit this fact and enforce the low-rankness of the solution through the parametrization $X = V^\top V$ \cite{burer2003nonlinear}.
Here, $V$ belongs to $\mathbb{R}^{k\times n}$ and $k$ satisfies the condition $k(k+1)/2>n$ \cite{boumal2016nonconvex}. This parametrization yields to a formulation of the SDP problem \eqref{eq:noncvx_continuous_form}, whereas the global value remains unchanged. 
Although, the new formulation is non-convex, there is actually a \emph{quid pro quo}: the conic constraint in \eqref{eq:continuous_form}, $X\succeq 0$, is automatically given through the parametrization $V^\top V$, which is the key reason that leads to more efficient approaches for solving SDPs: handling a PSD constraint per iteration requires an eigenvalue decomposition of $n \times n$ matrices per iteration, leading to a $O(n^3)$ overhead per iteration. 



% \textcolor{magenta}{
% Besides, the constraint in \eqref{eq:continuous_form} translates to $V \in (\text{Sph}^{k-1})^{n}$ ( the $n$-product of $k-1$ spheres); namely, each column vector $v_j$ satisfies $\|v_j\|_2 = 1$.}



==> ICML20-AAAI21/Proofs_Algorithm_2/ourApproach.tex <==
\section{Our approach}
Let
\begin{equation}\label{eq: g_i}
\begin{split}
    g_i &= \sum_{j< i} c_{i j} \hat{v}_j  + \sum_{j> i} c_{i j} v_j,
\end{split}
\end{equation}
and $y_i = \|g_i\|_2$. So, the usual mixing method is defined through the relation
\begin{equation*}
\begin{split}
    y_i u_i &= - g_i,
\end{split}
\end{equation*}
(where $u_i$ corresponds to update in the inner cycle of the vector $v_i$). The modification of the algorithm that we are proposing, it can be described with the following two steps
\begin{equation*}\label{eq:twoSteps}
\begin{split}
    u_i = - \frac{g_i}{y_i}, \hspace{10 pt} \text{ and } \hspace{10 pt} 
    \hat{v}_i = \frac{u_i - \beta v_i}{\|u_i - \beta v_i\|}.
\end{split}
\end{equation*}
For brevity's sake, define $w_i = \|u_i - \beta v_i\|$. 

So this leads us to the relation
\begin{equation}\label{eq:recursion}
    w_iy_i\hat{v}_i  = -g_i -\beta y_i v_i,
\end{equation}
for all $i \in [n]$.

==> ICML20-AAAI21/Proofs_Algorithm_2/random_thoughts.tex <==
\section{Random thoughts}
Using the projector operator from the previous theorem and letting $\nabla f(V) = 2VC$ we get the following characterization of the Riemannian gradient.
\begin{equation*}
    \mathrm{grad}f(V) =  2 \begin{bmatrix}g_1 - \langle v_1, g_1 \rangle v_1, \ldots, g_n - \langle v_n, g_n \rangle v_n  \end{bmatrix},
\end{equation*}

where $g_i = \sum_j C_{i,j} v_j$. Now using characterization \ref{lemma:decreasing} and the maps \eqref{eq: Z},  we know that 

\begin{equation*}
\begin{split}
    f(Z_i(V))&-f(Z_{i+1}(V))\\
    &= 2 g_i^\top \left(v_i + \frac{g_i+ \beta v_i \|g_i\|}{\| g_i+ \beta v_i \|g_i\|\|} \right)\\
    &\ge 2\left( g_i^\top v_i + \frac{\|g_i\|^2+ \beta \|g_i\| g_i^\top v_i}{\|g_i +  \beta v_i \|g_i\|\|}\right)\\
    &\ge 2\left( g_i^\top v_i +  \frac{1}{(1 + \beta)} \left( \|g_i\| + \beta v_i^\top g_i\right)\,\right)\\
    &=\frac{2}{(1+\beta)\|g_i\|} \left( \|g_i\|^2 + (1+2\beta) (g_i^\top v_i)\|g_i\|\right).
\end{split}
\end{equation*}

By Cauchy Schwarz inequality $(g_i^\top v_i) \le \|g_i\| $, so 

\begin{equation*}
\begin{split}
    f(Z_i(V))&-f(Z_{i+1}(V))\\
    &=\frac{2}{(1+\beta)\|g_i\|} \left( \|g_i\|^2 + (1+2\beta) (g_i^\top v_i)\|g_i\|\right)\\
    &\ge \frac{2}{(1+\beta)\|g_i\|} \left( \|g_i\|^2 + (1+2\beta) (g_i^\top v_i)^2\right)\\
    &\ge \frac{2}{(1+\beta)\|g_i\|} \left( \|g_i\|^2 - (g_i^\top v_i)^2\right)\\
    & \ge \frac{ \|\mathrm{grad}f(V)_i\|_2^2}{(1+\beta)\|g_i\|}.
\end{split}
\end{equation*}

Notice that $\|g_i\| \le  \sum_j|C_{i,j}| \|v_j\|_2 =  \sum_j |C_{i,j}| \le \|C\|_\infty$. Then 

\begin{equation}\label{eq:objective}
\begin{split}
    f(Z_i(V))&-f(Z_{i+1}(V))\ge \frac{\|\mathrm{grad}f(V)_i\|_2^2}{(1+\beta)\|C\|_{\infty}},
\end{split}
\end{equation}

where $\mathrm{grad}f(V)_i$ is the $i$th coordinate of the gradient. Now if we use the \texttt{mixing method++} the matrix $V$ changes at each iteration of the inner loop to $Z_{i+1}(V)$, making harder the comparison with the actual gradient at the initial point $V$. 

So we may assume that we update  the matrix $V$ after we finish the inner loop. Thus, using the previous relation we finally get 
\begin{equation*}
\begin{split}
    f(\hat{V})-f(V)&\ge \frac{\sum_i\|\mathrm{grad}f(V)_i\|_2^2}{(1+\beta)\|C\|_{\infty}}\\
    &= \frac{\|\mathrm{grad}f(V)\|_F^2}{(1+\beta)\|C\|_{\infty}}
\end{split}
\end{equation*}

From the previous relation is easy to see that we still have the following guarantees, the algorithm converges to stationary points, let $\{V^0, V^1, \ldots, V^N, \ldots\}$ the sequence matrix of the algorithm after the initial state, so if $f_{low}$ is a lower bound for the problem then
\begin{equation*}
\begin{split}
    \infty > f(V^0)-f_{low}&\ge f(V^0)-f(V^N)\\
    &=\sum_{k=0}^{N-1} f(V^k)-f(V^{k+1})\\
    &= \frac{1}{(1+\beta)\|C\|_{\infty}} \sum_k \|\mathrm{grad}f(V^k)\|_F^2,
\end{split}
\end{equation*}
since the sum is upper-bounded, $\|\mathrm{grad}f(V^k)\|_F^2 \to 0$ as $k\to \infty$. Using that $V^k$ contains an stationary point and by continuity of the norm we get $\mathrm{grad}f(\bar{V}) = 0$, so $\bar{V}$ is an stationary point. 


==> ICML20-AAAI21/experiments.tex <==
 \clearpage
\section{Experimental Results}
\subsection{Experiment Settings}
$\beta$ is in the following set: $\{-0.4,-0.2,0,0.2,0.4,0.6,0.8,1,1.2,1.4\}$.

Besides fixed $\beta$, we use the following adaptive values for beta.
\begin{itemize}
    \item Adaptive 1: $\beta_t=\frac{t}{t+3}$
    \item Adaptive 2: $\beta_t=\beta_{init}\cdot \frac{1-\frac{t}{T}}{(1-\beta_{init}+\beta_{init}(1-\frac{t}{T}))}$. The maximum number of iterations $T$ is known as a priori. For $\beta_{init}$ we use two values: 0.3 and 0.9.
\end{itemize}
\subsection{Erdos Random Graph}
The benchmarks are random graphs $G(n,p)$, where $n$ is the number of vertices and $p$ is the possibility of every two vertices having an edge. I tried four $n,p$ pairs (from sparse to dense): $(4000,0.001)$, $(4000,0.01)$, $(4000,0.05)$, $(2000,0.15)$. The termination threshold  $\varepsilon=1e-4$. Since I don't know the optimum of the SDP problem, I used the lowest function value I have ever seen from using all betas as the optimum (In fact, the largest beta (1.4) always gave the minimum function value compared with other betas). 

From the plots I have two observations:
\begin{itemize}
    \item The acceleration is more obvious on sparse graph and almost invisible on dense graph.
    \item Although the acceleration is not shocking, one good thing is, adding a reasonable beta ($<1.5$) seems to have no harm to the converged function value. Actually adding a beta improved the minimum function value compared with the algorithm without beta.
\end{itemize}
\begin{comment}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/4000_0001.png}
    \caption{MAXCUT on G(4000,0.001), $nnz\%=0.001$}
    \label{fig:my_label}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/4000_001.png}
    \caption{MAXCUT on G(4000,0.01), $nnz\%=0.01$}
    \label{fig:my_label}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/4000_005.png}
    \caption{MAXCUT on G(4000,0.05), $nnz\%=0.05$}
    \label{fig:my_label}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/2000_015.png}
    \caption{MAXCUT on G(2000,0.15), $nnz\%=0.15$ }
    \label{fig:my_label}
\end{figure}
\subsection{Gset Group}
\end{comment}
Benchmark source: \text{"https://www.cise.ufl.edu/research/sparse/matrices/Gset/index.html"}.

%The results are in Figure \ref{fig:g1}, \ref{fig:g27}, \ref{fig:g27}, \ref{fig:g58}, \ref{fig:g62} and \ref{fig:g65}.

Observations:
\begin{itemize}
    \item On different graphs the best $\beta$ is different.
    \item The accelerations on this group of benchmarks are more obvious than these on the Erdos random  graphs. 
\end{itemize}

\begin{comment}


\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.3\linewidth]{figures/G1.png}
  \captionof{figure}{MAXCUT on G1}
  \label{fig:g1}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.4\linewidth]{figures/G1shape.png}
  \captionof{figure}{G1: n=800, dense, $nnz\%=0.06$}
  \label{fig:g1s}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.2\linewidth]{figures/G27.png}
  \captionof{figure}{MAXCUT on G27}
  \label{fig:g27}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.4\linewidth]{figures/G27shape.png}
  \captionof{figure}{G27: n=2000, dense, $nnz\%=0.01$}
  \label{fig:g27s}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.3\linewidth]{figures/G58.png}
  \captionof{figure}{MAXCUT on G58}
  \label{fig:g58}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.4\linewidth]{figures/G58shape.png}
  \captionof{figure}{G58: n=7000, dense, $nnz\%=0.0024$}
  \label{fig:g58s}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.3\linewidth]{figures/G62.png}
  \captionof{figure}{MAXCUT on G62}
  \label{fig:g62}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.4\linewidth]{figures/G62shape.png}
  \captionof{figure}{G62: n=7000, sparse, $nnz\%=0.0006$}
  \label{fig:g62s}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.3\linewidth]{figures/G65.png}
  \captionof{figure}{MAXCUT on G65}
  \label{fig:g65}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=.4\linewidth]{figures/G65shape.png}
  \captionof{figure}{G65: n=8000, sparse, $nnz\%=0.0005$}
  \label{fig:g65s}
\end{minipage}
\end{figure}

\subsection{MaxSAT benchmarks}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/maxsat/maxcut-140-630-07-1.png}
    \caption{MAXSAT on maxcut-140-630-0.7-1.cnf, $n=140$, $m=1260$, $nnz\%=0.128$, dense}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/maxsat/s2v220c1200-1.png}
    \caption{MAXSAT on s2v220c1200-1.cnf, $n=220$, $m=1200$, $nnz\%=0.05$, dense}
    \label{fig:my_label}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/maxsat/scpclr10_maxsat.png}
    \caption{MAXSAT on scpclr10\_maxsat.cnf, $n=210$, $m=721$, $nnz\%=0.3$, super dense}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/maxsat/scpclr13_maxsat.png}
    \caption{MAXSAT on scpclr13\_maxsat.cnf, $n=715$, $m=4810$, $nnz\%=0.716$, super dense}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.65]{figures/beta_vs_cond.png}
    \caption{Optimal beta vs condition number of $C$ on 33 instances}
    \label{fig:my_label}
\end{figure}
\end{comment}




\subsection{Comparison on 4 Methods}
In this subsection, we compare 4 variants of accelerated Mixing methods:
\begin{itemize}
    \item Method 1 (Original method): 
    
    $\hat{V}_i=-Normalized(\sum_{i<j}C_{ij}V_j+\sum_{i>j}C_{ij}\hat{V}_j+\textcolor{red}{\beta V_i})$
    \item Method 2: 
    
    $\hat{V}_i=-Normalized(\textcolor{red}{Normalized}(\sum_{i<j}C_{ij}V_j+\sum_{i>j}C_{ij}\hat{V}_j)+\textcolor{red}{\beta V_i})$
    
    \item Method 3: Use an auxiliary matrix $X$ (Note that since $X$ and $V$ always have the same direction, we don't have to store $X$).
    
    $\hat{X}_i=(\sum_{i<j}C_{ij}V_j+\sum_{i>j}C_{ij}\hat{V}_j+\textcolor{red}{\beta X_i})$
    
    $\hat{V}_i=Normalized(X_i)$
    \item method 4: Adding momentum only after updating all coordinates, i.e.,
    
    $\hat{V}_i=-Normalized(\sum_{i<j}C_{ij}V_j+\sum_{i>j}C_{ij}\hat{V}_j)$ for $i$ in $\{1,...,n\}$
    
    $\hat{V}=Normalized{(\hat{V}-\textcolor{red}{\beta V})}$
    

\end{itemize}

I define the "\textbf{Acceleration ratio}" as follows:

Let the function value finally reached by $\beta=0$ be $f_0$ which uses $n_0$ iterations. Then for each method on each instance, I looked at the result given by the optimal $\beta$, let $n_{\beta}$ be the number of iterations at which the function value just reaches $f_0$. Then the "\textbf{Acceleration ratio}" is defined by $\frac{n_0}{n_{\beta}}$.

The results for distribution of optimal beta and the acceleration ratio are as follows.


\begin{figure}[h!]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/beta_vs_nnz_m1.png}
  \captionof{figure}{Distribution of optimum beta of Method 1}
  \label{fig:g62}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/acc_vs_nnz_m1.png}
  \captionof{figure}{Acceleration Ratio of Method 1}
  \label{fig:g62s}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/beta_vs_nnz_m2.png}
  \captionof{figure}{Distribution of optimum beta of Method 2}
  \label{fig:g62}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/acc_vs_nnz_m2.png}
  \captionof{figure}{Acceleration Ratio of Method 2}
  \label{fig:g62s}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/beta_vs_nnz_m3.png}
  \captionof{figure}{Distribution of optimum beta of Method 3}
  \label{fig:g62}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/acc_vs_nnz_m3.png}
  \captionof{figure}{Acceleration Ratio of Method 3}
  \label{fig:g62s}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/beta_vs_nnz_m4.png}
  \captionof{figure}{Distribution of optimum beta of Method 4}
  \label{fig:g62}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1.1\linewidth]{figures/acc_vs_nnz_m4.png}
  \captionof{figure}{Acceleration Ratio of Method 4}
  \label{fig:g62s}
\end{minipage}
\end{figure}

\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
Methods & MAXCUT & MAXSAT        \\ \hline
M1      & 1.64   & 2.02          \\ \hline
M2      & 4.76   & 3.89          \\ \hline
M3      & 7.48   & 2.63          \\ \hline
M4      & 1.58   & 1.56 \\ \hline
\end{tabular}
\caption{Average Acceleration ratio on 4 methods}
\end{table}
